Slice Agent: Identifying and Isolating Slices in Shared Open Radio Unit

Network Slice as a Service (NSaaS) is a key enabler of Beyond Fifth Generation (5G) and Sixth Generation (6G) networks, supporting next-generation applications such as extended reality (XR), immersive services, and the tactile Internet. These networks must provide native support for slice-aware services across the entire Radio Access Network (RAN), including the Radio Unit (RU), Distributed Unit (DU), Central Unit (CU), and transport segments (fronthaul, midhaul, and backhaul). However, uplink slicing identification in shared Open-RUs (O-RUs) presents a fundamental challenge because the Open-DU (O-DU) handles scheduling, and the O-RU does not inherently know which uplink data belongs to which slice. In MultiPoint-to-MultiPoint (MP2MP) fronthaul scenarios, this limitation is further exacerbated by synchronization and timing constraints, which necessitate that the O-RU process control messages and the encapsulated data be delivered with ultra-low latency. To address this issue, we propose a slicing agent embedded in the O-RU that identifies slices and segregates uplink data into slice-specific enhanced Common Public Radio Interface (eCPRI) packets. Our design employs a pipeline architecture with dedicated paths for time-sensitive, flexible slicing, enabling slice isolation and prioritization. When implemented on an Field-Programmable Gate Array (FPGA), the agent processes each packet in 2 clock cycles, supporting up to 3822 slices per slot. Experimental results validate the approach, showing its feasibility, scalability, and high-performance capabilities for real-time, slice-aware uplink processing in Beyond 5G and 6G Open RAN deployments.

==> ToDo.tex <==
Deadline para submissão dia 13/02

Deixar as alterações em azul

Lista de atividades que precisam ser realizadas antes da submissão:

%%%%%%% Título e Autores

DONE! 1) Adicionar nome e instituição do Flávio --> Flávio

%%%%%%% Abstract

DONE! 2) Alinhar o abstract de acordo com a introdução --> Cristiano

%%%%%%% Introduction

DONE! 3) Melhorar primeiro e segundo parágrafo da Introdução --> Cristiano

DONE! 4) Melhorar a escrita dos itens III e IV das contribuições --> Cristiano

DONE! 5) Precisa de um parágrafo destacando os resultados impactantes do trabalho --> Cristiano

%%%%%%% Background

DONE! 6) Adicionar referências dos orgão padronizadores --> Flávio

DONE! 7) Melhorar a descrição cronológica da evolução da RAN --> Flávio

DONE! 8) Atualizar Figura 1 alterando BBH para BBU --> Flávio

DONE! 9) Adicionar um texto indicando que o 3GPP sugere/escolhe a Option 2 --> Flávio

DONE! 10) Melhorar a subseção "Network slicing", destacando os conceitos fundamentais --> Flávio

%%%%%% Related Work

DONE! 11) Reestrutura a seção escrevendo os artigos em uma ordem cronológica para evitar repetições --> Cristiano Ps. Essa reestruturação não foi feita, mas uma descrição do motivo da "repetição" foi adicionada.

12) Adicionar referências atuais, de 2025 -->

DONE! 13) Adicionar referência do CO-DBA --> Cristiano

DONE! 14) Melhorar a descrição do problema de sincronismo --> Cristiano

DONE! 15) Adicionar os trabalhos que apresentam a visão do O-RAN na rede de transporte ---> Flávio

DONE! 16) Arrumar a argumentação de pq queremos identificar o slice no fronthaul?  "transport only elements only need to route or forward packets..." --> Cristiano

%%%% Slice Agent architecture

DONE! 17) Rever essa frase "The \ac{LLS} plays a crucial role in meeting fronthaul requirements." --> Flávio

DONE! IT 18) Reescrever a frase "However, in the uplink flow, \ac{O-RU} is responsible for identifying each slice and packing the New Radio data with the correct tag." --> Flávio

DONE! 19) Aumentar o texto da Figura 3 --> Cristiano

DONE! 20) Arrumar o texto para destacar que suportamos 2 tipos de slices, com uma grande quantidade de slices para cada um desses tipos --> Flávio

21) Pensar como podemos adicionar a ideia dos buffers na Figura 4 --> Deixar assim!!

DONE!! 22) Como identificamos os slices para colocar as TAGs? --> 

DONE! 23) Revisar a Figura 6 --> Cristiano

DONE! 24) Aumentar fonte da Figura 7 --> Cristiano

%%%% Performance evaluation

DONE !! 25) Ajustar vários detalhes na Figura 9 --> Cristiano

DONE! 26) Disponibilizar um repositório --> Cristiano

DONE!! 27) Revisar as fontes da Figura 10 --> Cristiano

DONE! 28) Explicar melhor como foi feita a alocação de PRBs no experimento --> Flávio

DONE! 29) Exlicar melhor os 2 tipos de slices, URLLC e eMMB? --> Flávio

30) Salvar a Figura 11, 12 e 13 em PDF --> deixar assim

DONE! 31) Explicar "Como seria isso? Em que cenário é possível manter 30 PRBs para 1 símbolo apenas?" --> Flávio

DONE! 32) Explicar o resultado da Figura 12, como está vinculando isso às amarras de tempoxfrequencia previstos nas normas 3GPP. Talvez seja interessante clarificar --> Flávio

DONE! 33) Detalhar melhor o cenário, por exemplo, de qual Banda estamos falando? FR1 ou FR2? --> Flávio

%%%% Colclusion

DONE !34) Discutir o caráter prático --> Flávio


==> old/sections_old/architecture.tex <==
\section{\sigla{} Architecture}
\label{sec:prop}

This section introduces the multi-radio and  multi-hop LoRa communication architecture called of \sigla{}. First, we describe a global view of the \sigla{} architecture. Next, we detail each layer of the architecture.

\subsection{Network model and scenario}

%\dlr{pode iniciar falando novamente de app rural que precisam ser implamtadas em uma área grande e com processamento em tempo real. Dai vai ser necessário uma rede loramesh coom baixo capex e opex.}
Agriculture plays vital importance in developing an agricultural country, where rural modernization emerges as a solution to improve farming, field, and producers' issues \cite{asin201250}. For instance, Smart agriculture refers to modernizing traditional methods \cite{gondchawar2016iot}. Among smart agriculture, applications stand out:
\begin{inparaenum}[($i)$]
    \item Applications to improve wine quality inspect soil moisture and trunk diameter in the vineyards. These features provide the development of vigorous vines and, consequently, a good harvest.
    \item Greenhouse applications manage microclimate conditions for the production of fruits and vegetables. These applications can avoid a microclimate conducive to \brown{developing} diseases in the plant and promote cultivation success.
    \item Golf course irrigation in dry areas reduces the water used by improving irrigation and lowering costs.
    \item Meteorological station network applications control weather conditions providing information and avoiding disasters.
    \item Compost application \brown{controls} humidity and temperature levels in vegetable matter found on farms, enabling better quality control for animal feed.
\end{inparaenum}
In this context, smart agriculture requires monitoring on a large scale with low cost and real-time data collection.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/landscape-v3.pdf}
    \caption{Network scenario overview}
    \label{fig:scenario}
\end{figure}

We consider a scenario composed of $n$ IoT devices and a gateway deployed over a large-scale rural area, as shown in Figure \ref{fig:scenario}. \brown{Each IoT device could act as a client and relay node in this scenario.} IoT devices act as \brown{clients} to collect environment data and send it to a gateway considering a multi-hop and multi-radio LoRa communication. IoT devices deployed between the client and gateway could act as a relay node based on routing decisions. The gateway forwards these incoming messages using an IP network to the targeting application server for further operations, such as analytic systems. For instance, the application server could consider a machine-learning algorithm to provide precision dairy farming information. Therefore, plants and animals get precisely the treatment they need in a data-driven fashion.


\subsection{Multi-LoRa network architecture}

The \sigla{} architecture provides a reference model for implementing multi-radio and multi-hop LoRa communication for large-scale IoT deployment in rural areas. \sigla{} architecture consists of four layers: Physical, MAC, Network, and Application, as shown in Figure \ref{fig:multiarquitetura}. 
Specifically, the Physical layer considers the LoRa® radio provided by Semtech \cite{dantas2021Survey}.
For upper layers, there are some expected features. For instance, the MAC layer must ensure an efficient  transmission scheme over multiple radios. Furthermore, the Network layer is responsible for forwarding the routing data to route the data with lower signaling overhead and half-duplex communication. Finally, IoT applications can be built at the Application layer. In the following, we describe each layer of our architecture.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/arch.pdf}
    \caption{\sigla{} network architecture overview}
    \label{fig:multiarquitetura}
\end{figure}

%\subsubsection*{\textbf{Physical Layer}} 
\textbf{Physical Layer} refers to the physical medium in which the communication will occur. Each radio considers Sender and Receiver buffers responsible for receiving data from the MAC layer sending it via the LoRa radio, obtaining data from another LoRa radio, and forwarding it to the MAC layer. For Lora Radio, we consider the LoRa® wireless technology \cite{raza2017low}. The radio means the Semtech chipsets used in any architecture in public, private, or hybrid networks, offering long-range, low power consumption, and secure data transmission. LoRa provides connectivity for the IoT devices to the Gateway for further operations. Unlike other wireless systems that use Frequency Shifting Keying (FSK) modulation for low power consumption, LoRa is based on Chirp Spread Spectrum (CSS) modulation. \brown{Moreover, LoRa maintains the same low power characteristics as FSK modulation but significantly increases the communication range \cite{dantas2021Survey}.} 

LoRa radio considers a half-duplex communication scheme, \ie, it cannot receive and transmit signals simultaneously \cite{dantas2021Survey}. However, half-duplex communication causes a collision of data packets or the inability to send packets on the same radio channel, \ie, packet collision problem. In this sense, multiple radios can mitigate this problem, reducing the collision rate because using the channel to send a packet is decreased. Therefore, multiple radios must consider the frequency multiplexing technique. It is statistically possible to reduce the collision rate since the use of the channel to send a packet is reduced by up to 50\% by fragmenting the data transmitted by both interfaces simultaneously. The frequency multiplexing control algorithm is responsible for the access control layer to the medium, discussed in the following.

%\subsubsection*{\textbf{MAC Layer}}

%LoRaWAN considers ALOHA as a MAC protocol, which does not perform well when traffic load or node density increases, due to interference and packet collisions \cite{cotrim2020lorawan}. The MAC layer of LoRaWAN is designed to work in a star topology, allowing only one hop between the IoT devices and the LoRaWAN gateway. ALOHA protocol might also not perform very well for multi-hop communication between IoT devices. In addition, t
%However, the access layer to the middle of this architecture will be responsible for managing the proposed multi-channel radio system to optimize latency and reduce collisions.
%The fragmentation of the information into several packets to transfer over multiple interfaces must result in a packet header more extensive than the payload, reducing the transmission efficiency.

\textbf{MAC Layer} must efficiently manage the access control layer of multiple radios and controls the synchronization between IoT devices that want to transmit \cite{babaee2018improved}. Therefore, it is essential to design the MAC layer to enable multi-hop and multi-radio LoRa communication as \brown{simple} as possible. In this way, the MAC layer considers the Multiplexer, Demultiplexer, and Carrier sensing modules. Moreover, the MAC layer is responsible for assessing whether the wireless medium is available to transmit packets using the Carrier sensing module. We consider the Listen Before Talk (LBT) communication model, where a radio transmitter first senses its radio environment before it starts a transmission \cite{dantas2021Survey}. LBT can be used by a radio device to find if a network the device is allowed to operate on or to find a free radio channel to work. \blue{Distinct from the MAC layers implemented in the traditional TCP/IP networks, the MAC layer does not consider any algorithm for handling collisions.} In our architecture, the application layer is responsible for managing collisions for two reasons: (\textit{i}) to keep the medium access control as simple as possible with low overhead; and (\textit{ii}) the applications consider the request and reply communication model, allowing the application to verify the packet delivery and retransmission in case of packet loss. 
%\dlr{falta explicar o multiplexer!}

The MAC layer considers the frequency diversity transmission scheme to send signaling packets from the routing protocol, allowing verification of the Radio Signal Strength Indicator (RSSI) value for each radio independently \cite{babaee2018improved}. \brown{This verification is because the frequency diversity transmission scheme enables all radios to transmit the same information simultaneously.} Moreover, signaling packets are tiny packets, and their fragmentation into two packets would result in a packet header larger than the valid information. Specifically, the data fragmentation into several packets to transfer over multiple interfaces must result in a packet header more extensive than the payload, reducing the transmission efficiency. However, we consider the frequency multiplexing scheme for sending packets containing application data, where the data is partitioned between the two available interfaces to be sent simultaneously. Moreover, the MAC layer considers the Demultiplexer to receive the packets through the available radio interfaces, verify the received data, and concatenate them into a single packet using the sequential number as a reference. Therefore, this packet is forwarded to the network layer. If one packet fragment is not received, the entire packet is drooped and not sent to the upper layer.


%\subsubsection*{\textbf{Network Layer}} 
\textbf{Network Layer} is responsible for forwarding the data to its final address within the network. This layer consists of the Routing algorithm, Routing table, Neighbor table, Scheduling, and Packet relaying. The Neighbor table on each node consists of the following 4-tuple: node address, sequence number, metric, and priority. Specifically, the node address means the address of the neighboring node. The sequence number denotes the last message received, used to compute the packet loss ratio. The metric represents the link quality of the neighboring address, such as RSSI or packet loss ratio. Moreover, the priority means the application priority that this client is configured to handle, \eg, it is used by the packet scheduling module. In this context, each node must \brown{update a neighbor's} table based on collected information from application packets and signaling messages. For instance, as soon as an application packet is not sent after a specified timeout period, \brown{the Routing algorithm module will send a signaling message} to ensure that a node is not dropped from a neighboring node's Routing table. 

Each node also has a Routing table composed of the following 6-tuple: destination, next-hop, distance, sequence number, metric, and priority. Specifically, destination means an address for a given route. The next-hop denotes the address required to reach the destination. The distance is the number of hops to reach the destination address used to discard the package if it exceeds this number to avoid loops. The sequence number means the number of the last received application packet from the destination used to compute the packet loss for this route. The filed metric represents the link quality between the destination address and its final hop. Finally, the priority means the application preference that this client is configured to handle, which the Scheduling module can use. It is fundamental to highlight that this architecture is not designed for a specific routing protocol, and thus we define a set of default fields for routing and neighbor tables. Therefore, these tables can be extended to add new fields, depending on the protocol needs.


The Packet relaying module is responsible for receiving the application packet or signaling message from the MAC layer and \brown{delivering} it to the corresponding module. The Packet relaying module updates the Neighbor table for each received application packet or signaling message in terms of control information. Moreover, it updates the Routing table for each signaling message during the route discovery process. The Packet relaying module delivers the packet to the application layer as soon as it addresses it in the application packet. Otherwise, it provides the Scheduling module to forward the packet to its final address within the network.

The Routing algorithm module is responsible for defining the route to reach the destination address and forwarding the data to its final address within the network. The Routing algorithm maintains the Routing table on each node by adding, updating, and removing routes based on the routing protocol and sending signaling messages. For example, the Routing algorithm could forward the data packet to its last address within the network based on the Routing table. The routing protocol for this type of network must be designed keeping in mind the topology changes over time. Moreover, the available bandwidth of LoRa radio is limited and should not be wasted on protocol decisions and header traffic. Therefore, it is required to provide a routing protocol that meets this multi-radio and multi-hop LoRa architecture's characteristics, such as the packet size limitation that leads to the need for lower signaling overhead and \brown{the use} of half-duplex communication. Based on \brown{table of neighbo} default information, the routing decision could be based on hop count, packet success, and link quality. Ad hoc algorithms define routes based on \brown{fewer} hops unless the packets' success rate falls below a specific limit. A wide range of ad hoc protocols, such as the Babel routing protocol (RFC 8966) \cite{rfc18966}, rely on the available information on the neighbors and routing tables used in our architecture.

It is essential to consider key application requirements individually rather \brown{than in a} one-fits-all solution. In this sense, the Priority module works with queues to prioritize packet transmission based on application priority to efficiently meet the required quality for each IoT application. The architecture supports any number of queues, where we define three queues as a default value, namely, low, normal, and priority queue. The Packet relaying module enqueues a packet into the corresponding queue based on the application priority. By default, we define that the Signal packet has low priority due to its static characteristics in its nodes. We specify the scheduling policy to consume the priority packets first to send to the MAC layer.

%\subsubsection*{\textbf{Application Layer}} 
\textbf{Application Layer} might coexist \brown{with} multiple applications with different quality requirements in large-scale rural IoT scenarios. It is essential to transmit data applications over LoRa radio with delays and throughput requirements with higher coverage. We define three levels of priority as default, \ie, 1, 2, and 3, to represent high, medium, and low application priority, respectively \cite{dawaliby2019network}. A high priority group requires low latency and message transmission intervals and low tolerance to data loss. However, a medium priority group requires high reliability and low latency but is lower than the high priority. Finally, a low priority is those with a high delay tolerance.

The Application layer must implement the reliability mechanism depending on the application requirements since the MAC layer only senses the physical medium without detecting collisions. The application considers the request and replies communication model, allowing the application to verify the packet delivery and retransmission in the case of packet loss. 


\section{\sigla{} Prototype}
\label{sec:Prototype}

This section presents the prototype for the \sigla{} architecture. We detail the hardware and the packet format based on the Babel routing protocol. After, we discuss the four main phases of operation of the architecture.

We developed a hardware prototype for physically implementing the \sigla{} architecture \brown{consisting} of hardware and software implementation, as shown in Figure \ref{fig:Prototype}. 
Each node shares the same hardware structure and main firmware. In terms of hardware implementation, each node is composed of an Espressif Esp32 microcontroller (dual-core 32-bit LX6 microprocessor, operating at 240 MHz and performing at up to 600 DMIPS, Ultra-Low-Power co-processor, 520 KB SRAM, 448 KB ROM), two LoRa radios SX1276, and energy source with a capacity of 2100 mAh. We implemented the MAC, routing, and application layer protocols on device firmware using the C programming language in software implementation. Specifically, we implemented the LBT communication model at the MAC layer, the Babel routing protocol (RFC 8966) at the network layer, and Modbus at the application layer. 
%\dlr{acho que era bom colocar informação de processamento e memória disponível} - \lrp{é suficiente ?}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/prototipo.pdf}
    \caption{Prototype Overview}
    \label{fig:Prototype}
\end{figure}



%\dlr{Foi usado esse endereço para ficar compatível com endereço da rede, e sem a necessidade de uma entidade para atribuir endereço}

%Based on the node address size, the network structure consists of a maximum number of 4.294.967.296 ($2^{32}$) %\lrp{Aqui  tem um furo, usei 4bytes para o endereço\\ pois tinha o mac do UC como referência. no caso pensamos em colcar enderço sequencial podemos conectar esses 4bi de devices, não faz sentido isso} IoT devices.

We designed a protocol to deploy our prototype by considering the limitations of a LoRa radio to exchange control and data information. In this sense, we adapted the Babel routing protocol (RCF 8966) \cite{rfc18966} to our prototype since it is largely used and easily implemented. For instance, we adapted the packet format to the size of the LoRa frame, \ie, 256 bytes. This size involves considering only 4 bytes for each address, \ie, source, destination, and next-hop, while babel considers 16 bytes for each IPv6 address or 16 bytes for each IPv4 address. Therefore, the packet header of \sigla{} has 16 bytes, while the packet header of the Babel routing protocol has 44 to 60 bytes considering IPv6 address or 60 bytes considering IPv4 address. This issue increases the packet payload and avoids packet fragmentation. Figure \ref{fig:pacote} depicts the \sigla{} packet format with 16 bytes of header and 240 bytes for payload. We consider the following fields as a packet header: 



%the packet format is based on the Babel routing protocol (RCF 8966) \cite{rfc18966} adapted to the size of the LoRa frame, \textit{i.e.}, 256 bytes. 
%Moreover, we defined a new protocol due to no existing standard protocol for multi-radio and multi-hop for LoRa communication.

\begin{itemize}
    \item Time to Live (TTL) [1 byte]: means the packet “lifetime”, which can be seen as the number of hops allowed before a node drops the message.
    \item Size [1 byte]: is the length of the packet, \ie, header and payload.
    \item Source and destination addresses [4 bytes]: identifiers of the node that originated the packet and the intended packet destination address.
    \item Next-hop address [4 bytes]: is the identifier of the next node, which the packet should be forwarded, to reach the destination address.
    \item Sequence [1 byte]: means the global message counter to determine the packet loss ratio and duplicated. Moreover, it is used to demultiplex the fragments received by the two radio interfaces, where both fragments must have the same sequence to be grouped.
    \item Type [1 byte]: is an ASCII character \brown{that} describes the payload content. $r$ means route message, $h$ denotes hello message, $m$ means more significant data, $l$ represents less significant data, and so on.
\end{itemize}

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/packet.pdf}
    \caption{\sigla{} packet format}
    \label{fig:pacote}
\end{figure}

%\dlr{no babel, o next-hop fica no payload e isso vai requerer maior processamento. esse pacote foi adaptado para poder caber dentro do tamanho do frame lora, pois os formatos de pacotes de protocolos de roteamento adhoc para TCP/IP são mt grande. Com isso, vai haver mt fragmentação.}




%As a packet header, we consider the following fields: Time to Live (TTL), Size, source address, destination address, next-hop address, sequence, and type. Specifically, TTL means the packet “lifetime”, which can be seen as the number of hops allowed before a node drops the message. Size is the entire length of the packet (header + data). Source and destination addresses mean a 4-byte identifier of the node that originated the packet and the intended packet destination address. The next-hop address is the 4-byte of the IoT node to which the packet should be forwarded to reach the destination address. Sequence means the global message counter, which determines the packet loss ratio. Moreover, it is used to demultiplex the fragments received by the two radio interfaces, where both fragments must have the same sequence to be grouped. Type is an ASCII character, which describes the payload content. For instance, $r$ means route message, $h$ denote hello message, $m$ means more significant data, $l$ denote less significant data, and so on. Data is the payload of the packet.

The Babel routing protocol includes the next-hop information as a packet payload, introducing additional processing at the relay node to get such vital information. \blue{In this case, we consider the next-hop address within the packet header.} Each node has a unique 4-byte identifier based on the least significant bytes of the MAC address of the hardware, which is used to guarantee this individual address. We used this identifier to keep the compatibility with the MAC address. We define the broadcast address as 0xFFFFFFFF. It is fundamental to highlight that we can have a larger node address size at the cost of reducing the payload size. As soon as a node joins the network for the first time, it needs to go through four main phases: (\textit{i}) Discovery, (\textit{ii}) Learning, (\textit{iii}) Forwarding, and (\textit{iv}) Convergence before starting the packet routing. We discuss these phases in the following subsections.

%\dlr{ver como e onde encaixar essa parte.} The routing protocol used as a reference was that described by RFC8966, also known as the Babel Protocol. It was adapted to the architecture proposal of this work, since originally Babel specification is for a TCP/IP network. Some of its characteristics, such as simplicity of implementation and robustness, were determining factors for choosing this as the basis for implementation. \dlr{we need to describe more Babel}


\subsection{Discovery phase}


%During the discovery phase, the IoT node broadcasts a hello message to present itself to its neighbors and hears other hello messages being broadcasted in its interval. In this sense, each IoT node can discover its neighbors and add them to the neighbors tables. The hello message has a size of 16 byte, which contains only the header information as a tuple (1, 16, source address, 0xFFFFFFFF, 0xFFFFFFFF, sequence number, h). 
 
 
Figure \ref{fig:discovery} shows the sequence diagram for the Discovery phase, enumerating each sequence. During the Discovery phase, the Routing algorithm creates a hello message (1) at each time interval to present itself to its neighbors, transmitted by a given LoRa radio with low priority (2). The hello message has a size of 16 \brown{bytes}, which contains only the header information as a tuple ($1$, $16$, $source$ $address$, $0xFFFFFFFF$, $0xFFFFFFFF$, $sequence$ $number$, $h$). In addition, the hello message has a TTL with the value $1$ to avoid flooding, which means that each hello message is broadcasted only to one-hop neighbors. Therefore, a hello message can be seen as a signaling message addressed to all neighbors using the broadcast address. Moreover, it loads the message sequence number and application priority information to form the node's Neighbor table.



Each IoT node discovers its neighbors by hearing the hello messages being broadcasted by the node neighbors (3). The Packet relaying analyzes the hello message (4) and adds/updates the neighbor information in the Neighbor table (5). We implemented the Neighbor table as a list with the following features: Node address, Packet success, Metric, and Priority, wherein each entry has 8 bytes. Finally, after a defined time limit, all neighboring nodes already know about the existence of a new node, or at least a minimum number of neighbors discovered, then the node starts the Learning phase.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/Seq_diagram_1.pdf}
    \caption{Sequence diagram for the Discovery phase}
    \label{fig:discovery}
\end{figure}

\subsection{Learning phase}


%During the learning phase, a node shares its routing table with its neighbors and listens to the routing table message broadcasted by the neighbors. It analyzes the routing table message and updates its routing table. In this way, the node learns about the neighbors of his neighbors, that is, us with several hops away. Specifically, the routing table message has a size of s-byte (\ie, header and payload), which contains the header information as a tuple (1, s, source address, 0xFFFFFFFF, 0xFFFFFFFF, sequence number, r). In addition, we include the routing table as the payload data. We implemented the routing table as a list with the following information: Destination, Next hop, distance,  sequence number, metric, and priority, where in our implementation each entry has a size of 8-byte. Due to the limited packet size (\ie, 240 bytes of data), the routing table message is limited to 30 routes (\ie, 8 bytes for each route). After discovering more than 30 routes, a node needs to send several messages to share its entire routing table.

Figure \ref{fig:learning} shows the sequence diagram for the Learning phase, enumerating each sequence. During this phase, the Routing algorithm creates a routing message (1) to share its Routing table with its neighbors (2), transmitted by a given LoRa radio with low priority (3). The routing message contains the header information as a tuple ($1$, $s$, $source$ $address$, $0xFFFFFFFF$, $0xFFFFFFFF$, $sequence$ $number$, $r$), and the Routing table as the payload data. The routing message has a size of s-byte (\textit{i.e.}, header and payload). Due to the limited packet size (\textit{i.e.}, 240 bytes of data), the routing message is limited to 30 routes (\textit{i.e.}, 8 bytes for each route). Therefore, a given IoT node with more than 30 routes needs to send several messages to share its entire Routing table created by the MUX/DEMUX (4-5).



The Packet relaying module analyzes the message by overhearing a routing message from a given IoT node (6). The route information within the message is compared with all existing routes in the Routing table. As a result, the Packet relaying adds the new route to its table, updates a current route with a new or better metric, or eliminates the route, as it has a better route or the route refers to the local address of the nodes (7). Each IoT node learns about its neighbors and reaches a given node within the network. We implemented the Routing table as a list with the following information: Destination, Next-hop, distance, sequence number, metric, and priority, wherein each entry has a size of 8-\brown{bytes}. The Learning phase is probably never complete, as new nodes may appear at any time. After a determined time configured as a parameter on each node in the network, the node enters the Forwarding phase.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/Seq_diagram_2.pdf}
    \caption{Sequence diagram for the Learning phase}
    \label{fig:learning}
\end{figure}

\subsection{Forwarding phase}

Figure \ref{fig:forwarding} shows the sequence diagram for the Forwarding phase. The Application collects the information and sends it to the Scheduling to send the information to the destination node (1). Whenever a given IoT node wants to send the collected information to a given destination node, it sends the data information to the Scheduling. The Scheduling creates the data packet and enqueues a packet into the corresponding queue based on the application priority (2). The Routing algorithm consumes the packets from the priority queue based on First In First Out. It encapsulates the information to reach the destination based on requests to the Routing table (3). 



MUX/DEMUX fragments the data packet into several packets  to transfer over multiple interfaces (4-5). Moreover, MUX/DEMUX sends the data packet to the Packet relaying (6), which analyzes the destination address within the packet header, \textit{i.e.}, a 128-\brown{bytes} packet transmitted over one radio interface is composed of 16 bytes of header and 112 bytes of payload. When the packet is transmitted over two radio interfaces, it is segmented into two packets. In this case, each packet contains 16 bytes of header, and the payload is equally partitioned into 56 bytes. After, Packet relaying sends the data packet to the Application as soon as the packet reaches the destination node (9). Otherwise, it sends the data packet to the Scheduling (7) to enqueue a packet into the corresponding queue based on the application priority (8). The algorithm continues until the packet reaches the destination node. Finally, we consider the frequency multiplexing scheme for sending packets containing application data, where the data is partitioned between the two available interfaces to be sent simultaneously.


\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\textwidth]{figures/Seq_diagram_3.pdf}
    \caption{Sequence diagram for the forwarding phase}
    \label{fig:forwarding}
\end{figure}

%In the forwarding state, a node discovered a certain number of neighbors and learned about the network to be considered a good route. This state must be considered the normal operational state of a network node, since it can now be used to send packet and to forward packets addressed to the nodes to which it has routes. 

\subsection{Convergence phase}

The Convergence phase is the integration of the three first phases. This convergence implies that every node is aware of a route to all other nodes in the network. In this sense, a node in the network knows the address of each node and the next-hop address to reach the destination address, but it does not know the entire network topology. This knowledge reduces the memory required to maintain a Routing table and the time needed for convergence. Therefore, it is unnecessary to store the complete route for all nodes, only the neighboring node's information to reach the final node.

\brown{The four phases designed are fundamental for supporting large-scale IoT and guaranteeing the efficiency of the Multi-LoRa architecture.} In this context, we present a performance evaluation of the Multi-Lora architecture based on our prototype in the next section.





==> old/sections_old/background.tex <==
\section{Background}



==> old/sections_old/backup.tex <==
\section{Introduction}

%apresentar smart farm e aplicaçõe semelhantes. Importância de monitoramento para essas aplicações e que não tem como colocar infra.

% ler aritog: https://www.mdpi.com/1424-8220/20/15/4273
% https://www.mdpi.com/1424-8220/20/13/3632
%http://www.libelium.com/resources/top_50_iot_sensor_applications_ranking/


The recent explosion of the Internet of things (IoT) technology is dramatically changing society through disruptive technologies in new sets of verticals and applications \cite{buzzi2016survey}.
Smart farms/agriculture and rural electrical power distribution for the smart grid are only a few examples of intelligent environment IoT verticals \cite{taneja2019connected, kulatunga2017opportunistic, visconti2020development}. 
IoT plays vital importance in supporting farmers in response to the global food challenge of feeding more than 9 billion people in 2050 and the sustainability and competitiveness challenges. IoT devices could be deployed over huge areas in the farmlands to detect and collect soil information, precise climate, animal tracking, and information referred to growth or diseases of the cultivated crops \cite{visconti2020development}.
For example, in Brazil, there are farms with thousands of hectares for cotton planting. In this case, cotton packages are left on the farm for long periods, and they can catch fire with humidity below 12\%. Therefore, monitoring the farmland avoids financial losses and extensive burning to increase agriculture efficiency in continental countries with an agricultural vocation.

IoT technologies help to produce high-quality fruits and vegetables in sufficient quantities to satisfy food requirements while maintaining competitive costs \cite{visconti2020development}. The collected data must feed decision-support systems to provide precision dairy farming information, and thus plants and animals get precisely the treatment they need in a data-driven fashion. The improvements in productivity and environmental sustainability rely on the analytics' accuracy, which strongly depends on the amount and timeliness of the data collected \cite{kulatunga2017opportunistic}. Therefore, it is essential to provide a data acquisition in farms where network connectivity is a constraint. The data acquisition solution must ensure timely, efficient, and reliable communication and performance longevity for IoT devices deployed over huge farmlands \cite{kulatunga2017opportunistic}. 

To capture the long-range communication requirements, innovative long-range technologies, such as Low Power Wide Area Network (LPWAN) \cite{raza2017low}, is attracting attention from both academy and industry through promising capabilities in a broad area, operating on unlicensed frequency bands, low power consumption, and throughput tailored to IoT application verticals \cite{haxhibeqiri2018survey}. In this context, the Long-Range Wide Area Network (LoRaWAN) architecture is considered the most adopted LPWAN architecture for its ubiquitous connectivity capacities in outdoor use cases \cite{matni2020experimenting}. 
%\dlr{In particular, LoRa physical layer is a proprietary spread spectrum modulation based on the robust Chirp Spread Spectrum (CSS) by Semtech \cite{lyu2019achieving}. Based on the LoRa physical layer, the LoRa Alliance \cite{alliance2015white} defined the higher layers and network architecture of the Long-Range Wide Area Network (LoRaWAN) \cite{croce2018impact}.}
LoRaWAN architecture considers a single-hop communication between the IoT device and gateway over several channels, forming a star network topology. IoT devices broadcast messages for neighbor gateways, which forwards the message to the application server through an existing IP network. Based on such architecture, LoRaWAN provides connectivity to IoT devices deployed over a vast area by employing a control access mechanism with less complexity at the cost of low throughput \cite{qadir2018low}. Specifically, LoRaWAN achieves nearly 2-5 km of coverage range in urban areas and about 45 km in rural areas \cite{8783184}. Therefore, the low-power, low-cost, and long-range properties provided by LoRaWAN allow devices to spread and move over large geographic areas \cite{8217061}. 

% J. M. Marais, R. Malekian and A. M. Abu-Mahfouz, "Evaluating the LoRaWAN Protocol Using a Permanent Outdoor Testbed," in IEEE Sensors Journal, vol. 19, no. 12, pp. 4726-4733, 15 June15, 2019, doi: 10.1109/JSEN.2019.2900735. Esse trabalho pode ser usado para citar uma cobertura menor da rede lorawan (práticamente 5 km de raio e não os 45 teóricos)

Even though LoRaWAN provides about \textcolor{red}{45 km} of coverage in rural areas, it might not be sufficient for data acquisition in farms, which has hundreds of kilometers. The deployment of more gateways could be integrated into the network ecosystems to increase the coverage area. However, deploying gateways lead to high Capital Expenditure (CAPEX) and Operational Expenditure (OPEX), including the cost of a gateway, of its leasing, maintenance, etc. \cite{matni2020lorawan}. Therefore, a multi-hop network plays an essential role in applications requiring extensive network deployment, which is not addressed by LoRaWAN architecture \cite{cotrim2020lorawan}. It is possible to consider a multi-hop LoRa communication among the gateways, IoT devices, or both to increase the coverage area \cite{cotrim2020lorawan}. However, it is not convenient, cheap, or even feasible to deploy multiple gateways in a farm scenario. Several IoT devices might be deployed with a LoRa radio in a farm scenario to monitor the environment, which might also work as a relay. Therefore, a multi-hop LoRa architecture between IoT devices should provide communication to the gateway for any IoT device deployed over huge areas in the farmlands to send real-time data samples to analytic systems \cite{kulatunga2017opportunistic}. 

In this context, it is important to design an efficient LoRa architecture to enable multi-hop communication for large scale IoT deployment in rural areas. In addition, multiple radios can be used to mitigate the collision caused by the half-duplex nature of LoRa radio, and thus the collision rate can be reduced because the time of using the channel to send a packet is decreased. However, it is essential to design an efficient transmission scheme over multiple radios at higher layers (MAC and routing layers).
The MAC layer must efficiently manage the access control layer of multiple radios. Therefore, it is also important to design the MAC layer to enable multi-hop and multi-radio LoRa communication.
Hence, it is required to provide a routing layer that meets the characteristics of this multi-radio and multi-hop LoRa architecture, such as the limitation of the packet size that leads to he need for lower signaling overhead and use of half-duplex communication.
It is essential to consider key application requirements individually rather than a one-fits-all solution. Therefore, it is important to design an efficient architecture to transmit data over LoRa radio for applications with different delay and throughput requirements with higher coverage over large scale rural IoT scenarios. To the best of our knowledge the state-of-the-art works does not present an architecture that integrate multi-radio and multi-hop LoRa communication in an efficient solution.

%\textcolor{red}{Melhorar o link entre esses parágrafos}

% pelo que entendi essa característica é mais uma motivação para se propor uma arquitura. Logo, não deveria vir antes do parágrafo anterior?

%LoRa radio considers a half-duplex communication scheme, \ie, it cannot receive and transmit signals simultaneously. Therefore, half-duplex causes collision of data packets or the inability to send packets due to the same radio channel, \ie, packet collision problem. In this sense, multiple radios can be used to mitigate this problem, and thus the collision rate can be reduced because the time of using the channel to send a packet is decreased. However, it is essential to design an efficient transmission scheme over multiple radios at higher layers (MAC and routing layers), since LoRa has a lower data rate. The fragmentation of the information into numerous packets to transfer over multiple interfaces must result in a packet header more extensive than the payload, reducing the transmission efficiency.

%% agora começa a falar de LoRaWAN --- acho que precisa criar uma ordem para introduzir LoRaWAN e LoRa e não ficar intercalando.

% pelo que entendi essa característica é mais uma motivação para se propor uma arquitura. Logo, não deveria vir antes do parágrafo anterior?

%LoRaWAN considers ALOHA as a MAC protocol, which does not perform well when traffic load or node density increases, due to interference and packet collisions \cite{cotrim2020lorawan}. The MAC layer of LoRaWAN is designed to work in a star topology, allowing only one hop between the IoT devices and the LoRaWAN gateway. ALOHA protocol might also not perform very well for multi-hop communication between IoT devices. In addition, the MAC layer must efficiently manage the access control layer of multiple radios. Therefore, it is important to design the MAC layer to enable multi-hop and multi-radio LoRa communication.

% repensar a ordem desses parágrafos e tb se precisa ser tão detalhada a introdução assim !!

%The network layer is responsible for forwarding the data to its final address within the network. The routing layer is in charge of maintaining the routing tables on each node, adding, updating, and removing routes only when the quality changes. However, the available bandwidth of LoRa radio is limited, and should not be wasted on protocol decisions and header traffic. Hence, it is required to provide a routing layer that meets the characteristics of this multi-radio and multi-hop LoRa architecture, such as the limitation of the packet size that leads to he need for lower signaling overhead and use of half-duplex communication.

%There might coexist multiple applications with different Quality of Service (QoS) requirements in a large scale rural IoT scenarios. This scenario leads to new challenges in order to design an efficient algorithms based on application priority for decision making in order to efficiently meet the required QoS for each IoT application. It is essential to consider key application requirements individually rather than a one-fits-all solution. Therefore, it is important to design an efficient architecture to transmit data over LoRa radio for applications with different delay and throughput requirements with higher coverage over large scale rural IoT scenarios. To the best of our knowledge the state-of-the-art works does not present an architecture that integrate multi-radio and multi-hop LoRa communication in an efficient solution.

%pergunta de pesquisa: como transmitir serviços com maior alcance e diferentes requisitos de atraso e vazão para aplicações IoT em ambientes rurais?

%\dlr{This scenario leads to the need to design an efficient architecture to enable multi-hop communication for large scale IoT deployment in rural areas.} Arquitetura com pouca complexidade e baixo custo.


With this challenge in mind, we propose a multi-radio and multi-hop LoRa communication architecture to increase the coverage and QoS for large scale IoT deployment in rural areas, called \sigla{}. It provides a reference for the implementation of communication networks based on the physical layer LoRa. \dlr{describe the work.} We introduce an experimental case study to analyze the performance of the proposed architecture.

The main contributions of this article can be summarized as follows: 
\begin{inparaenum}[$i)$]
    \item We propose a \sigla{} architecture to enable multi-radio and multi-hop LoRa communication between IoT devices running applications with monitoring QoS requirements.
    \item We perform real experiments to introduce the impacts and benefits of \sigla{}, where the results show that \sigla{} can effectively mitigate the challenges related to multi-hop communication over LoRa for large scale IoT deployment in rural areas to increase the connectivity.
\end{inparaenum}    

\begin{itemize}
    \item \sout{não temos mais classes de app.}

    \item \sout{Protocolo BABEL do wifi simplificado para LoRa.}

    \item redução do cabeçalho para aumentar o tamanho do pacote, pois o radio esta sempre escultando.

    \item \sout{Não tem eficiência energética, podemos falar em energy harvesting. Podemos falar que é mais importante transmitir para algumas aplicações do que salvar energia.}

    \item dois radios para aumentar a capacidade de transmissão e menor delay.

    \item \sout{possível de fazer uma transmissão ou encaminhamento com prioridade.}

    \item \sout{possível ter multiplos radios LoRa.}
\end{itemize}

%propondo uma arquitetura para loramesh que considera a camada fisica do LoRa e adiciona novos modulos. essa arquitetura é agnostica em termos de qlqr modulo e aplicação. Conseguimos rodar um DNP3 e IoT, etc.

The rest of the article is organized as follows. Section~\ref{sec:relatedworks} introduces the related work about the multi-hop LoRa communication. Section~\ref{sec:prop} presents \sigla{} for improving the coverage of LoRa communication in large scale IoT scenarios. Section~\ref{sec:metrics} introduces an experimental case study to analyze the performance of the proposed architecture. Finally, Section~\ref{sec:conc} concludes the work and introduces the future works.












%O protótipo de hardware para implementar fisicamente a arquitetura da rede modelada consiste em um sistema microprocessado, composto por hardware, software e interface de rádio apresentado na Figura 24. Esse sistema é composto por três dispositivos que compartilham a mesma estrutura de rádio e firmware principal, apenas com configurações de conexões externas diferindo.



%A rede de comunicação, mesmo com a falha do sistema elétrico que ela monitora e usa como fonte de alimentação, não deixará de funcionar, pois cada dispositivo na rede tem capacidade de ser alimentado por uma bateria que manterá seu funcionamento em momentos de falha. Com a rede de comunicação funcionando, a localização exata do ponto de falha da rede elétrica é feita de maneira mais rápida. O uso de dois canais em rádio independentes (duas frequências) faz com que diminua a colisão e também que se garanta links de backup no caso da perda de um canal. Não é possível utilizar a mesma frequência com SF diferente, pois os rádios dos nós baseados no circuito integrado SX1276 ou SX1262 apenas reconhecem um fator de espalhamento espectral (SF) configurado. Assim, a proposta de Zhu et al. (2019), em que ele usa apenas um canal (frequência) com diferentes fatores de espalhamento para implementar as técnicas de multiplexação não será possível de se implementar. Seria necessário basear toda a proposta em outro circuito integrado, o SX1301, capaz de trabalhar com diferentes fatores de espalhamento espectral ao mesmo tempo. Porém, o custo seria muito elevado. Hoje, ele é utilizado apenas nos gateways da rede LoRaWAN (FSK; LORA; LORA, 2017).

%\dlr{descrever o hw usado, os protocolos, o formato da msg.}





%Na Figura 13, é apresentada a estrutura básica da arquitetura, dividida em camadas aderentes ao modelo OSI (Open Systems Interconnection).
%O modelo apresentado será detalhado em cada uma de suas camadas e implementação nos tópicos a seguir.

%4.1.1 Camada Física

%A camada física do modelo proposto, refere-se ao próprio meio físico no qual a comunicação irá ocorrer. Como a arquitetura foi projetada tendo como premissa o uso da tecnologia sem fio LoRa®, já discutida anteriormente, esse será o meio físico utilizado. Os rádios LoRa® comunicam-se utilizando o esquema de comunicação half-duplex, ou seja, não podem receber e transmitir sinais simultaneamente. Um outro ponto a retomar é a colisão de pacotes de dados ou a impossibilidade de transmitir pacotes devido ao uso do mesmo canal de rádio, i.e., os problemas de colisão de pacotes. A solução proposta para minimizar esse problema foi a implementação de uma camada física que faça uso de dois canais de rádio e que utiliza as técnicas de multiplexação de frequência, apresentadas na revisão teórica e propostas pelo trabalho de Majumdat al. (2017) para outras tecnologias de redes sem fio. Assim, estatisticamente pode-se reduzir o índice de colisões, pois o tempo de uso do canal para enviar um pacote, é reduzido em até 50\%, visto que o dado é particionado e enviado por ambas as interfaces simultaneamente. O algoritmo de controle da multiplexação de frequência, será de responsabilidade da camada de controle de acesso ao meio e serão discutidas a seguir.

%4.1.2 Camada de Acesso ao Meio (MAC)

%Esta camada assegura o acesso ao meio, assim como controla a sincronização entre duas entidades que queiram transmitir. Ela é a responsável por avaliar se o canal de rádio que se pretende utilizar está livre. Diferente das camadas MAC implementadas em redes TCP/IP,  não serão implementados algoritmos para o tratamento de colisões por meio de envio de pacotes RTS (Request to Send) e CTS (Clear to Send), como sugerido por Islam (2019). Essa responsabilidade será da aplicação por dois motivos: manter o controle de acesso ao meio o mais simples possível e com menor overhead e também devido a todas as aplicações que farão uso da rede implementarem o modelo de pergunta e resposta, o que, permite verificar a entrega e a retransmissão dos pacotes de dados caso não ocorra a resposta devido a uma colisão . No entanto, a camada de acesso ao meio dessa arquitetura será responsável por gerenciar o sistema de múltiplos canais de rádio proposto para a otimização da latência e diminuição das colisões. 

%O esquema de transmissão Diversidade de Frequência em que a mesma informação é transmitida por ambos os canais ao mesmo tempo, será utilizada para o envio de pacotes de sinalização do protocolo de roteamento, permitindo, assim, verificar as métricas de qualidade de link  que usa o valor do Radio Signal Strength Indicator (RSSI) para cada um dos canais de forma independente. Também se justifica o uso dessa técnica por se tratarem de pacotes de tamanho bastante reduzidos, e sua fragmentação em dois pacotes ocasionaria em um header de pacote maior que a informação válida. Já o esquema de Multiplexação de Frequência, onde o dado a ser transmitido é particionado entre as duas interfaces disponíveis e enviado simultaneamente, será utilizado para o envio de pacotes contendo dados da aplicação.

%Assim como o condicionamento do dado de sinalização ou de informação da aplicação, a camada também deverá receber os pacotes através de ambas as interfaces de rádio, realizar a verificação dos dados recebidos e concatená-los em um único pacote usando como referência o número sequencial de pacote, que é o mesmo no cabeçalho de ambos os fragmentos. Esse pacote, será repassado para a camada de rede discutida na sequência. No caso de um dos fragmentos de pacote não ser recebido, o pacote inteiro é descartado e não é encaminhado para a camada superior.

%4.1.3 Camada de Rede

%Essa camada será a responsável pelo encaminhamento dos dados até seu endereço final dentro da rede Mesh. O protocolo de roteamento para esse tipo de rede precisa ser concebido tendo em mente a topologia de uma rede variável onde links entre os diversos nós, podem ser estabelecidos ou removidos. A largura de banda disponível e o desempenho dos nós Mesh são limitados e não devem ser desperdiçados com decisões de protocolo e com tráfego de cabeçalhos. Atualmente, existe um leque variado de protocolos e implementações Mesh que se encarregam de manter as tabelas de roteamento em cada nó como por exemplo o Destination Sequenced Distance-Vector Routing , adicionando, atualizando e removendo rotas apenas quando a qualidade delas altera-se, e, para isso, utilizam o processo de cálculo de métricas de qualidade. 
%Como apresentado anteriormente, existem vários algoritmos e protocolos de roteamento consolidados que foram implementados para redes baseadas em TCP/IP. Como a arquitetura de comunicação proposta não utiliza uma rede desse tipo, será necessário implementar um protocolo que atenda às características dessa arquitetura, como a limitação do tamanho do pacote em 256 bytes, necessidade do menor overhead de sinalização possível, uso de meio de comunicação half-duplex, entre outros. Assim, devido às suas características de simplicidade de implementação, robustez e eficiência, o protocolo de roteamento para redes Mesh baseadas em tecnologia LoRa®, criado para este trabalho, foi baseado no protocolo de roteamento RFC6126, também conhecido como Babel (CHROBOCZEK; SCHINAZI, 2018). 
%Nessa camada, também será implementada a técnica de priorização de pacotes através de três filas de envio: a fila de baixa prioridade, a fila normal e a fila prioritária, permitindo que seja possível a coexistência dos serviços. 


%4.1.3.1 Protocolo de Roteamento Desenvolvido 

%A seguir, serão apresentadas as características e funcionalidades do protocolo desenvolvido. O protocolo de roteamento utilizado como referência foi o descrito pela RFC6126, também conhecido como Protocolo Babel. Ele foi adaptado para a proposta da arquitetura deste trabalho, pois originalmente sua especificação é para uma rede TCP/IP. Algumas de suas características, como simplicidade de implementação e robustez, foram fatores determinantes para a escolha deste como base da implementação.

%4.1.3.2 Endereçamento

%Cada nó da rede, possui um endereço exclusivo de 4 bytes. Para garantir esse endereço exclusivo, optou-se por utilizar os bytes menos significativos do endereço MAC do hardware utilizado.  O endereçamento broadcast implica que as mensagens são enviadas para vários destinatários; esses destinos têm um endereço broadcast compartilhado de 4 bytes. Inicialmente, o único endereço broadcast é 0xFFFFFFFF, ou seja, transmissão limitada a todos os nós vizinhos.

%4.1.3.3 O Formato do Pacote 

%\begin{figure}[htb]
%    \centering
%    \includegraphics[width=0.5\textwidth]{figures/lora_mesh_frame.png}
%    \caption{\dlr{precisamo refazer.}}
%    \label{fig:pacote}
%\end{figure}
	
%O formato do pacote de dados apresentado no Quadro 9, é similar ao descrito na especificação original do protocolo Babel que serviu como base, apenas adaptando-se o tamanho dos campos à limitação imposta pelos rádios LoRa® e adicionando o campo “Salto” o qual é preenchido com o endereço do próximo nó a ser atingido para alcançar o destino final. Desta forma mantém-se o tamanho do dado fixo, diferente da versão original do protocolo, onde os primeiros bits do campo dado continham o endereço do próximo salto em caso de um pacote que necessitasse de vários saltos para atingir seu destino.

%Quadro 9 – Especificação do formato do pacote usado pelo protocolo de roteamento
%Byte 
%0	Byte 
%1	Bytes
% 2 - 5	Bytes
% 6 - 9	Bytes 
%10 -13	Byte 
%14	Byte 
%15	Bytes
%16 - 256
%TTL	Tamanho	Origem	Destino	Salto	Sequência	Tipo	Dado
% Fonte: Elaborado pelo autor com base na RFC6126.

%Onde:
%TTL: é o “tempo de vida”, ou seja, o número de saltos permitidos antes que a mensagem seja descartada por um nó;
%Tamanho: é todo o comprimento do pacote (cabeçalho + dados);
%Origem: é o endereço de 4 bytes do nó que originou a mensagem;
%Destino: é o endereço de 4 bytes do nó de destino pretendido;
%Salto: é o endereço de 4 bytes do próximo nó para onde o pacote deve ser encaminhado;
%Sequência: é o contador global de mensagens que determina a taxa de perda de pacotes, também usado para demultiplexar as os fragmentos recebidos pelas duas interfaces de rádio. Ambos fragmentos devem possuir a mesma sequência para serem agrupados;
%Tipo: é um caractere ASCII, que descreve o conteúdo da carga útil (por exemplo, r = pacote de rotas, h = pacote de hello, m = dados mais significativos, l = dados menos significativos);
%Dado: é o conteúdo da mensagem a ser interpretada pela camada de aplicação.

%4.1.3.4 Encaminhamento

%Uma tabela de vizinhos é gerada por mensagens regulares e mensagens de hello. Quando uma mensagem regular não é enviada após um período de tempo-limite especificado, um pacote hello será enviado para garantir que um nó não seja descartado da tabela de roteamento de um nó vizinho. Uma entrada na tabela de vizinhos consiste nos seguintes campos:
%Endereço: é endereço de 4 bytes do nó vizinho;
%Sequência: é o número de sequência da última mensagem recebida desse endereço usado para recalcular a perda de pacotes (descrito no tópico Métricas);
%Métrica: é uma representação de 0 a 255 da qualidade do link para o endereço vizinho;
%Protocolo: é o protocolo da aplicação de REI (DNP, Modbus ou NBR14522) que este cliente está configurado para tratar. Esta informação é usada para gerar uma tabela de protocolos por nós, o que garante que os dispositivos gateway saibam para qual nó deve ser enviada a requisição;
%SlaveAddress: é o endereço do dispositivo escravo associado ao nó (referente ao protocolo que o cliente está configurado).

%4.1.3.5 Pacote Hello

%Para evitar inundar a rede, os pacotes hello têm o campo TTL de 1, o que significa que eles são transmitidos por apenas um único salto. Ele também implementa um endereço multicast simples, de modo que qualquer vizinho imediato possa recebê-lo. Um pacote hello pode ser visto como qualquer pacote endereçado a todos os vizinhos usando o endereço multicast. Ele também carrega as informações de protocolo e slave address para formar a tabela de vizinhos do nó. 

%4.1.3.6 Tabela de Encaminhamento

%A tabela de encaminhamento (roteamento) em um nó da rede, consiste nos seguintes campos:
%Destino: é o endereço de 4 bytes do ponto final da rota;
%NextHop: é o endereço de 4 bytes do vizinho através do qual o ponto final pode ser alcançado;
%Distância: é o número de saltos do ponto final, usado para descartar o pacote caso ele ultrapasse este número, evitando assim loops;
%Sequência: é o número de sequência da última mensagem recebida do destino usada para recalcular a perda de pacotes;
%Métrica: é uma representação de 0 a 255 da qualidade do link entre o endereço de destino e seu salto final;
%Protocolo: é o protocolo da aplicação de REI (DNP, Modbus ou NBR14522) que este cliente está configurado para tratar;
%SlaveAddress: é o endereço do dispositivo escravo associado ao nó (referente ao protocolo que o cliente está configurado).

%A tabela de roteamento é gerada pelos nós que anunciam suas rotas para seus vizinhos. A publicação de rotas exige que pacotes maiores  com todas as rotas armazenadas em um nó, sejam transmitidos a fim de divulgar para seus vizinhos, quais os nós conhecidos e, portanto, sejam enviados com menos frequência do que pacotes hello. Além da tabela de roteamento, nessa tabela também está armazenada a informação de qual protocolo é tratado em cada nó, assim como seu endereço de escravo correspondente ao protocolo tratado. Assim, é possível fazer a relação do dispositivo escravo com o endereço de nó na rede Mesh permitindo que os nós gateways possam encaminhar o pacote externo à rede para o dispositivo escravo correto.

%4.1.3.7 Pacotes de atualização das tabelas de roteamento

%Assim como os pacotes hello, os pacotes de tabelas de roteamento têm um TTL de 1 e usam endereços multicast, ou seja, enviados apenas para vizinhos imediatos. Na recepção por um nó vizinho, esses dados são analisados e as rotas contidas são comparadas com todas as rotas existentes na tabela de roteamento do nó. Após comparar, o nó adiciona a rota à sua tabela, atualiza uma rota existente com uma nova ou melhor métrica ou elimina a rota, pois possui uma rota melhor ou a rota se refere ao endereço local dos nós.
%Devido ao tamanho limitado do pacote (240 bytes de dados), um pacote da tabela de roteamento é limitado a 30 rotas (8 bytes/rota). Após descobrir mais de 30 rotas, um nó precisa enviar vários pacotes para compartilhar toda a sua tabela de roteamento. 

%4.1.3.8 Métricas

%\dlr{a arquitetura é extensível para suportar qualquer métrica para decisão de roteamento, basta inlcuir a iformação na tabela de vizinhos.}

%Para a seleção de rota, um nó da rede usa duas métricas, a contagem de saltos e sucesso de pacotes. Um nó dá preferência ao menor número de saltos, a menos que a taxa de êxito dos pacotes caia abaixo de um determinado limite. 
%O sucesso do pacote como no protocolo Babel original, é calculado a partir do número de sequência no cabeçalho dos pacotes e é representado por um valor de 0 a 255. Se um nó perder um pacote do vizinho, o valor de sucesso do pacote será diminuído em 16, o que significa que após 16 pacotes perdidos, o sucesso do pacote será reduzido para 0.

%4.1.3.9 Estados dos Nós da Rede

%Quando um nó ingressa na rede pela primeira vez, ele precisa passar por vários estados antes de iniciar o roteamento de pacotes, estes estados são apresentados na Figura 14 e detalhados a seguir.

%Figura 14 – Estados de um nó ao ingressar na rede mesh
 
%Fonte: Elaborada pelo autor.

%	Estado de Descoberta: Durante a fase de descoberta, um nó transmite pacotes hello para se apresentar a seus vizinhos e ouve outros pacotes sendo enviados em seu intervalo, para que ele possa descobrir seus vizinhos e adicioná-los às tabelas de roteamento. Depois de um tempo limite definido ou um número mínimo de vizinhos descobertos, o nó entra na fase de aprendizado;
%	Estado de Aprendizado: Durante a fase de aprendizado, um nó compartilha sua tabela de roteamento com seus vizinhos e escuta os pacotes de roteamento enviados pelos vizinhos. Ele analisa os pacotes de roteamento conforme descrito acima e atualiza sua tabela de roteamento. Dessa forma, ele aprende sobre os vizinhos de seus vizinhos, ou seja, nós com vários saltos de distância. A fase de aprendizado provavelmente nunca está completa, pois novos nós poderão aparecer a qualquer momento. No entanto, após um certo tempo, configurado como um parâmetro em cada nó da rede, o nó entra no estado de encaminhamento;
%	Estado de Encaminhamento: no estado de encaminhamento, um nó descobriu uma certa quantidade de vizinhos e aprendeu sobre a rede para ser considerado uma boa rota. Esse estado deve ser considerado o estado operacional normal de um nó da rede, pois agora ele pode ser usado para enviar mensagens e retransmitir mensagens endereçadas aos nós para os quais possui rotas; 
%	Estado de Convergência: a convergência implica que todo nó tem conhecimento de uma rota para todos os outros nós da rede. Pode-se dizer que um nó da rede sabe o endereço de cada nó na rede e o endereço de salto para alcançar esse endereço, mas não conhece toda a topologia da rede. Isso reduz a memória necessária para manter uma tabela de roteamento e o tempo necessário para a convergência, pois não é necessário armazenar a rota completa para todos os nós, apenas a informação de qual deverá ser o nó vizinho utilizado para  alcançar o nó final;

%4.1.4 Aplicação

%A aplicação não faz parte da arquitetura desenvolvida, será a aplicação do usuário quem fará o envio e o recebimento de pacotes de dados. No caso, a proposta inicial da arquitetura prevê como aplicações o recebimento e o envio de pacotes dos protocolos de redes elétricas inteligentes, DNP3, Modbus e NBR 14522. 
%Finalizada a explicação de cada uma das camadas no modelo proposto, será explicado com maiores detalhes o protocolo responsável pelo roteamento dos pacotes entre os nós da rede.


%4.1.5 Estrutura de Rede

%A estrutura da rede é composta por um número máximo de 1024 dispositivos (dispositivos finais, roteadores e gateways) com suas interfaces de rádio, que transmite mensagens omnidirecionalmente, de modo que, em condições ideais, todos os nós devem receber todas as mensagens transmitidas por um nó vizinho. A limitação de 1024 dispositivos é devido ao número de entradas na tabela de roteamento que cada dispositivo conseguirá armazenar nesta primeira versão do protocolo. Como alternativa a essa limitação, pode-se realizar a clusterização da rede, como a proposta da Figura 15, que, para este modelo, irá consistir em configurar os nós da rede para trabalharem em um outro par de frequências, elegendo um outro dispositivo como nó roteador daquele cluster. 



No Quadro 10, pode-se observar os parâmetros da simulação configurados na ferramenta. A limitação do pacote de teste em 200 bytes dá-se por ser o tamanho máximo do dado alocado em um único pacote. Com as técnicas de múltiplos canais de rádio empregadas, essa limitação não existe (permite até 480 bytes), comportando assim o tamanho do maior pacote, no caso, 292 bytes do protocolo DNP3. Porém, para mantermos a mesma base de comparação, todos os demais testes serão realizados com esse tamanho de pacote.

Quadro 10 – Configurações da rede de testes no simulador do cenário de testes
PARÂMETRO	CONFIGURAÇÃO
Distância máxima da transmissão 	4 km
Tempo entre as requisições 	5 segundos
Tamanho do pacote DNP3	200 bytes
Tamanho do pacote Modbus	200 bytes
Tamanho do pacote NBR 14522	64 bytes pergunta / 200 resposta
Envio de pacote de rotas	A cada 2 minutos
Largura de Banda	125 kHz
Envio de pacote hello	A cada 1 minuto
Tempo de simulação	10 minutos
Fonte: Elaborado pelo autor.

Para a realização do teste físico real, os módulos de rádio LoRa® tiveram sua potência de transmissão reduzida através da configuração em registradores, além do sinal da antena atenuado fisicamente, forçando, assim, um alcance máximo de aproximadamente 4 metros verificados de forma empírica. Dessa forma, conseguiu-se reproduzir em escala reduzida (1:1000) a topologia da rede descrita no cenário de testes.


2 Caso Base Rede Sem Múltiplos Canais de Rádio e Priorização de Pacotes

Neste primeiro caso de teste, não foram habilitados nenhum dos mecanismos implementados na arquitetura para otimizar seu desempenho. No Gráfico 2, são apresentados na forma de histograma e na forma de diagrama de frequência cumulativa, os valores de latência para a requisição e as respostas dos nós configurados com o protocolo DNP3. Pode-se observar no cenário de testes da Figura 25, que para se alcançar esses nós, são necessários 3 saltos de roteamento. 
Gráfico 2 – Latência dos pacotes DNP3 nos testes realizados (SF = 7)
  \begin{figure*}[htb]
%\centering
%	\vspace*{-15mm}
 \begin{center}
\includegraphics[]{figures/teste_base.png}
  \end{center}
%\centering
%\vspace*{-15mm}
\caption{Protótipo de hardware}
\label{fig:loramesh}
\end{figure*}
Fonte: Elaborada pelo autor.


Pode-se observar que houve uma pequena discrepância entre a aplicação real e a simulação, se analisarmos os pacotes individualmente. Porém, o valor médio nos dois casos ficou em torno de 1198 ms (1198,44 ms na simulação e 1198,24 ms na aplicação real). O intervalo de confiança calculado ficou entre 1198,12 ms e 1198,76 ms.  Na simulação, ocorreu a perda de apenas um pacote dos 1000 pacotes enviados, já na aplicação real, três pacotes foram perdidos. Essa diferença pode ser explicada, pois o envio de pacotes de sinalização e rotas no simulador ocorre em instantes muito próximos para todos os nós. Todos eles foram instanciados quase que no mesmo instante. Já na rede real, os nós não iniciam seu funcionamento sincronizados. O jitter medido na simulação foi de 15 ms, e na aplicação real de 19 ms.


6.1.3 Avaliação do Impacto da Técnica de Priorização de Pacotes

O mesmo cenário de testes do tópico anterior foi mantido, porém, agora os pacotes DNP3 estão sendo enviados com prioridade alta, o que faz com que o mecanismo de filas priorize o tratamento desses pacotes. No Gráfico 5, é apresentado o comportamento da latência para os pacotes priorizados.
Gráfico 5 – Latência dos pacotes DNP3 com o mecanismo de priorização de pacotes
 
 \begin{figure*}[htb]
%\centering
%	\vspace*{-15mm}
 \begin{center}
\includegraphics[]{figures/teste_priorizacao.png}
  \end{center}
%\centering
%\vspace*{-15mm}
\caption{Protótipo de hardware}
\label{fig:loramesh}
\end{figure*}
Fonte: Elaborada pelo autor.


	Nas barras do histograma que representam a aplicação real, se comparadas ao cenário anterior (Gráfico 2), fica evidente a diminuição do jitter, que passou de 19ms para 10ms, comprovando que a priorização do pacote gera um melhor determinismo nas transmissões para aquela aplicação específica. O valor médio nos dois casos foi de 1198,50 ms na simulação e 1194,46 ms na aplicação real. O intervalo de confiança calculado ficou entre 1198,17 ms e 1194,64 ms. 


6.1.4 Avaliação do Impacto das Técnicas Multiplexação de Frequências 

Neste caso de teste, foram habilitados os mecanismos de diversidade de frequências (dois canais de rádio transmitindo simultaneamente o pacote segmentado), que foi implementado na arquitetura para otimizar seu desempenho, reduzindo o tempo de latência. O mecanismo de priorização de pacotes apresentado anteriormente não está habilitado. No Gráfico 6, são apresentados os valores de latência para a requisição e respostas dos nós configurados com o protocolo DNP3. 
Gráfico 6 – Latência dos pacotes DNP3 com o emprego da Técnica de Múltiplos Canais de Rádio
  \begin{figure*}[htb]
%\centering
%	\vspace*{-15mm}
 \begin{center}
\includegraphics[]{figures/teste_multiplexacao.png}
  \end{center}
%\centering
%\vspace*{-15mm}
\caption{Protótipo de hardware}
\label{fig:loramesh}
\end{figure*}
Fonte: Elaborado pelo autor.

Quando comparado ao caso original, em que, para alcançar o nó DNP3, são necessários os mesmos 3 saltos, a técnica múltiplos canais de rádio (multiplexação de frequências) reduz em 40\% a latência do envio de um pacote (BW = 125kHz). Se alterarmos a configuração de largura de banda para BW = 250 kHz, a redução de latência atinge 70\%, ficando em torno de 350 ms. Tempo esse bastante aceitável para uma rede Mesh com largura de banda limitada como a proposta pois fica dentro do timeout especificado para as aplicações de redes elétricas inteligentes. Nos dois cenários, por se tratar de uma rede de testes bastante pequena, não houve perda de pacotes, assim, é possível inferir que a redução de latência de pacotes diminui a possibilidade de colisões, principal causador da perda de pacotes. 


6.1.5 Avaliação do Impacto do Número de Saltos

Neste caso de teste, o cenário foi modificado, configurando a distribuição dos nós, de forma que para o pacote chegar ao seu destino deve ser retransmitido (roteado) por outros nós da rede. Esse cenário foi sendo alterado incrementando-se o número de saltos de roteamento como apresentado no Gráfico 7, onde são exibidos os valores médios de latência e perda de pacotes para cada caso sem o uso da técnica de múltiplos canais de rádio.

Gráfico 7 – Impacto do número de saltos na latência média e perda de pacotes (BW =125kHz e SF = 7)
 \begin{figure*}[htb]
%\centering
%	\vspace*{-15mm}
 \begin{center}
\includegraphics[]{figures/teste_saltos_base.png}
  \end{center}
%\centering
%\vspace*{-15mm}
\caption{Protótipo de hardware}
\label{fig:loramesh}
\end{figure*}
  Fonte: Elaborado pelo autor.

Já no Gráfico 8, são exibidos os valores médios de latência e perda de pacotes para o mesmo cenário descrito anteriormente, porém agora com a largura de banda alterada para 250 kHz e a utilização da técnica de multiplexação de frequência.
Gráfico 8 – Impacto do número de saltos na latência média e perda de pacotes (BW = 250kHz e SF = 7 e Múltiplos Canais)
  \begin{figure*}[htb]
%\centering
%	\vspace*{-15mm}
 \begin{center}
\includegraphics[]{figures/teste_saltos_multiplexacao.png}
  \end{center}
%\centering
%\vspace*{-15mm}
\caption{Protótipo de hardware}
\label{fig:loramesh}
\end{figure*}
Fonte: Elaborado pelo autor.

	Comparando-se os dois cenários, o primeiro sem otimizações e o segundo com otimizações presentes, percebe-se a diminuição considerável da latência e uma diminuição da perda de pacotes de 14\% para 4,7\%.  Porém também é evidente que a partir do quarto salto de roteamento, mesmo com as técnicas de otimização a rede começa a apresentar uma degradação de desempenho. Após a apresentação de alguns dos testes que validaram o comportamento do simulador de comunicação desenvolvido, será apresentado um estudo de caso que busca validar a integração das ferramentas no modelo de co-simulação.



==> old/sections_old/conclusion.tex <==
\section{Conclusion}
\label{sec:conc}

This article introduced \sigla{}, a multi-radio and multi-hop LoRa communication architecture, to enhance the coverage and service for large-scale IoT deployment in rural areas. The \sigla{} architecture was based on an ad hoc network topology to increase the coverage area. Moreover, we defined data multiplexing mechanisms in multiple LoRa radios to enhance throughput and decrease collisions. Furthermore, we determined small-scale and large-scale experiments considering three \sigla{} setups to evaluate the influence of the multi-radio and LoRa radio configurations. \blue{Specifically, \sigla{} reduced the delay by 60\% and packet loss by 2.9\% compared to different setups of \sigla{} on a small-scale physical testbed and large-scale simulation environment.} Hence, the results showed that the \sigla{} architecture effectively mitigates the challenges of multi-hop communication over LoRa for large-scale IoT deployment in rural areas to enhance connectivity. For example, the multi-hop characteristic improves the coverage area for a large-scale IoT deployment in rural areas. At the same time, the multi-radio decreases the half-duplex nature of LoRa radio.

Future work is being planned to evaluate the performance with multiplexing on a more significant number of radios and \brown{improve} routing algorithms. Moreover, we will analyze the \sigla{} prototype implementations considering reducing power consumption and serving remote rural areas without significant energy sources. \blue{We also plan to compare the performance of \sigla{} against existing multihop LoRa architectures.} \brown{Finally, we intend to develop a fault detection system to guarantee network reliability in remote areas such as large rural areas. This fault system will help to reduce operating costs for improve agriculture efficiency.}

%Nos testes  iniciais, apenas com a rede de comunicação proposta pode-se observar que, na comparação com o cenário base, foi evidenciado a diminuição do jitter (de 19ms para 10ms), o que comprova que o mecanismo de priorização do pacote gera um melhor determinismo nas transmissões para aquela aplicação específica e permite manter a taxa de transmissão dos pacotes mais constante. Se comparado ao caso base original, a técnica de multiplexação com múltiplos canais de rádio reduz em 40\% a latência do envio de um pacote, mantendo a mesma largura de banda. Se alterarmos a configuração de largura de banda para 250 kHz, a redução de latência atinge 70\%, ficando em torno de 350 ms, tempo esse bastante aceitável para uma rede Mesh com recursos bastante limitados como a proposta. Nos dois cenários com as técnicas, não houve perda de pacotes para a rede proposta com 8 nós e envio de pacotes a cada 5 segundos. Assim, pode-se inferir que a redução de latência de pacotes diminui a possibilidade de colisões, principal causador da perda de pacotes. Os resultados foram para uma rede de testes bastante reduzida, mas pode-se observar, através da comparação no primeiro cenário, que o comportamento do simulador de rede Mesh implementado é bastante próximo ao comportamento da implementação física da mesma rede. Já para os testes de impacto gerados pelo número de saltos de roteamento, no parâmetro latência o comportamento apresentado pelo simulador apresentou-se muito similar ao observado na rede real, porém no parâmetro perda de pacotes houve uma discrepância que variou de 2\% até 6\% entre o simulador e a rede real com o incremento dos saltos. Isso demonstra que esse deve ser um ponto de atenção para melhorias futuras no modelo de simulação.

%Ao fim da tese, pode-se destacar que o modelo da arquitetura e a implementação da rede de comunicação Mesh foram validados com sucesso. Entendeu-se, contudo, que sua aplicação tem limitações de uso, pois explora uma tecnologia com restrições de largura de banda para transmissão de dados, embora tenha custo relativamente baixo de implementação em larga escala, características de boa tolerância a interferências, podendo prover a conectividade mínima para uma rede inteligente rural, desde que bem dimensionada

==> old/sections_old/deletados.tex <==
we introduce the top 10 most popular IoT application verticals~\cite{asin201250}

Farms play an essential role in today's societies, both in their harvests and animals, by requiring to ensure proper environments and diets for animals and plants. \textit{smart animal farming} applications play an important role in this context~\cite{7724630}, where the most outstanding applications are: 
\begin{itemize}
    \item Hydroponics applications examine the exact state of cultivated plants, which is performed without the use of soil, the plants are fed through a nutrient solution. These applications make it possible to control the pH and electrical conductivity of the water, where the plants are grown, allowing for more intensive production.
    \item Offspring care applications measure the growing conditions of puppies on farms, ensuring healthy adult animals.
    \item Animal tracking applications find and identify animals in large stables, allowing greater control of animals by farmers.
    \item The toxic gas level application analyzes ventilation and air quality in farms. 
\end{itemize}

Agriculture also plays a vital importance in the development of an agricultural country. Therefore, agricultural modernization emerges as a solution to improve agriculture, field, and farmers' issues. \textit{Smart agriculture} refers to modernizing the current traditional methods~\cite{gondchawar2016iot}. Among the applications of smart agriculture stand out:
\begin{itemize}
    \item Applications to improve wine quality inspect soil moisture and trunk diameter in the vineyards. These features provide the development of vigorous vines and, consequently, a good harvest.
    \item Greenhouse applications manage microclimate conditions for the production of fruits and vegetables. These applications can avoid a microclimate conducive to the development of diseases in the plant, as well as promoting the success of cultivation.
    \item Golf course irrigation in dry areas reduces the amount of water used by improving irrigation and lowering costs.
    \item Meteorological station network applications control weather conditions providing information and avoiding disasters.
    \item Compost application control of humidity and temperature levels in vegetable matter found on farms, enabling better quality control for animal feed.
\end{itemize}

==> old/sections_old/evaluation.tex <==
\section{Performance Evaluation}
\label{sec:metrics}

\blue{This section describes the parameters used in our evaluation environment. Moreover, we introduce the performance metrics used to test \sigla{} architecture and determine a valid option to provide proof of concept of \sigla{} architecture.} We evaluate \sigla{} based on two complementary scenarios. The first is a small-scale physical, while the second is a simulation environment to analyze the scalability of the \sigla{} architecture. 



\subsection{Methodology}

We evaluated the \sigla{} prototype considering two approaches: a small-scale based on a physical testbed and a large-scale using \blue{a simulation} environment, as shown in Table \ref{tab:experiemtns}. The testbed results are investigated to calibrate the \blue{simulation} experiments and analyze the performance of \sigla{} in real experiments. Moreover, the \blue{simulation} experiments evaluated \sigla{} concerning delay and data delivery in a large-scale scenario. \blue{Furthermore, it is necessary to highlight that our simulation used the same source code prototyped in the testbed and available on GitHub\footnote{https://github.com/luciorp/multi-lora}.}

% Tirei pq achei repetitivo
%% In this sense, we assessed the \sigla{} prototype in the testbed and the emulation experiment, as shown in Table \ref{tab:experiemtns}.

We conducted the small-scale experiment on the 2nd floor of the Computer Engineering Department at UNISINOS. We deployed 8 IoT nodes (\ie, \brown{the} hardware prototype described in Section \ref{sec:Prototype}) organized in a grid topology of 3 $\times$ 3 in a controllable environment with a short field size of 8 $\times$ 12 meters. We consider the distance of 4 meters between each IoT node in such grid topology. It is fundamental to highlight that we reduced the radio range to 4 meters, decreasing the signal power. In this case, we reduced the radio range to carry out a small-scale experiment in a controlled environment. Moreover, we define a set of four packet sizes for the data packets, \ie, 32, 64, 128, and 256 bytes, where the packet header has 16 bytes, as expected for many rural applications that send data packets with different sizes.

% Based on such topology and radio configuration, each IoT node (\ie, source node) transmits data to LoRa Gateway over 1 to 3 hops.


%%% Escrever primeiro o que é diferente em cada cenário
 

%\lrp{Nessa análise levantou-se a taxa média de perdas para um tamanho de pacote de 128bytes  entregando mensagens a nós que  estavam a até 6 saltos. o setup foi  uma matriz iniciando  com 2x5 para 10 nós  4x5 para 20 nós, 6x5 para 30 nós, 8x5 para 40nós, 10x5 para 50 nós  e  10x10 para 100 nós.} 

\green{In our simulation environment, the routing packets are captured by a virtual network interface at the MAC layer and then redirected to the simulation model, which follows the methodology of VirtualMesh \cite{Staub2010}. The simulation model computes the network response according to the virtual network topology and the current position of the virtual nodes. The simulation occurs only in the physical medium, while all the other layers remain unchanged and work according to real hardware implementation. We define the propagation time of each packet based on the SX1276 datasheet\footnote{ https://www.semtech.com/products/wireless-rf/lora-core/sx1276} and \cite{moraes2022evaluation}. In this sense, it is possible to determine the collision of packets by analyzing the timestamp of each packet on a given receiving node. In this sense, packets with overlapping timestamps at a given node are considered collisions and consequently discarded.}

We designed the \blue{simulation} scenario to evaluate the \sigla{} prototype on a large-scale. We deployed 10 to 200 IoT nodes considering a field size of 40 $\times$ 80 km. Specifically, we organize the IoT nodes in a grid topology, \ie, 2 $\times$ 5,  10 $\times$ 5, 10 $\times$ 10, and 10 $\times$ 20 for 10, 50, 100, and 200 nodes, respectively, with a distance of 4 km between each IoT node and the Gateway at the center of such topology. \brown{Each packet was transmitted over 1 to 6 hops based on such topology and the routing protocols.} Moreover, each packet has 128 bytes, \textit{i.e.}, \brown{medium packet size, and is used} in real application scenarios \cite{HUU2020}. Finally, it is fundamental to highlight that the \blue{simulation} is essential to evaluate the scalability of \sigla{}, due to limited available IoT nodes in the testbed. Therefore, we implemented the \sigla{} protocol stack, where  the \blue{simulation} results have a similar behavior compared to testbed results, as our previous work showed in Prade et al. \cite{prade2020lora}. 



%We only considers collisions at the receiver node
%In addition, the simulation considers the \dlr{qual? quando chega dois pacotes no mesmo tempo em um nó relay ou destino, ambos são removidos, ou seja não é um path loss model} path loss model, which is regarded as suitable for rural data communication scenarios.

% We deployed 20 IoT nodes in a field size of 12 x 21 km, and in Scenario 2, we used 10 to 100 IoT nodes considering a field size of \dlr{xxx} km. Therefore, we defined a grid topology with a distance of 4 km between each IoT node and a LoRa Gateway on edge in both scenarios. Based on such topology, each IoT node (\ie, source node) transmits data to LoRa Gateway over 1 to 6 hops (Scenario 1) and 1 to 3 hops (Scenario 2). Moreover, for Scenario 1, we defined a set of four packet sizes for the data packets, \ie, 32, 64, 128, and 256 bytes.

%%% O que é comum para os 3 cenários 

We considered similar parameters for some essential characteristics for the small-scale (testbed) and large-scale (\blue{simulation}). For example, each IoT node sends a data packet to the LoRa Gateway and waits for an acknowledgment to send another data packet. \blue{In the end, each IoT node sends 1000 data packets since our goal is to evaluate the data delivered over a congested scenario.} Table \ref{tab:experiemtns} summarizes the main experimental parameters. We conducted experiments considering three setups: (\textit{i}) \textit{Multi-LoRa - Setup 1}, (\textit{ii}) \textit{Multi-LoRa - Setup 2}, and (\textit{iii}) \textit{Multi-LoRa - Setup 3}. 
\blue{Specifically, \textbf{Multi-LoRa - Setup 1} represents a multi-hop architecture with one LoRa radio configured with Spread Factor (SF) 7 and Bandwidth (BW) of 125 kHz, similar to the work presented by Diop and Pham \cite{mamour2019increased}. 
\textbf{Multi-LoRa - Setup 2} means a multi-hop architecture with two LoRa radios configured with SF 7 and BW of 125 kHz, where SF and BW values are chosen based on Diop and Pham \cite{mamour2019increased}. }
Finally, \textbf{Multi-LoRa - Setup 3} represents a multi-hop architecture with two LoRa radios configured with SF 7 and BW of 250 kHz. We increased the BW value to evaluate its impact because a higher BW value will afford to achieve an increased data transfer rate. Moreover, a low Time on Air (ToA) provides a shorter radio range and greater noise sensitivity \cite{dantas2021Survey}. 
%Specifically, the study of Diop and Pham represents the related work with a multi-hop architecture with one radio configured with Spread Factor (SF) 7 and Bandwidth (BW) 125 kHz. 


\begin{table}[!htb]
    \centering
    \caption{Parameters of evaluation for the \sigla{} architecture}
    %\scriptsize 
    %\footnotesize
    \begin{tabular}{l|c|c}
        \hline
        Characteristics & Small-scale (testbed) & Large-scale (\blue{simulation})  \\ \hline
        
        %% o que é diferente
        
        \rowcolor{gray!10} Number of nodes & 8 & 10-200 \\
        
        Field size & 8 x 12 (m) & 40 x 80 (km)  \\
        
        \rowcolor{gray!10} Topology &  4 m &  4 km  \\
        
%        Number of hops & 1-3 & 1-6 & 1-3 \\
        
        Packet size (bytes)  & 32, 64, 128, 256 &  128      \\ 
        
        %% o que é comum
         
        \rowcolor{gray!10} Number of Packets  & \multicolumn{2}{c}{1000}      \\
         
         & \multicolumn{2}{c}{Setup 1 (one radio with SF7 / 125 KHz)}      \\
         Multi-LoRa setups  & \multicolumn{2}{c}{Setup 2 (two radios with SF7 / 125 KHz)}      \\
         & \multicolumn{2}{c}{Setup 3 (two radios with SF7 / 250 KHz)}   \\  \hline
    \end{tabular}
    \label{tab:experiemtns}
\end{table}

We used the following two metrics to evaluate the performance of each setup, namely Packet Loss Ratio (PLR) and Average Packet Delay (APD). PLR $\in$ [0, 100] is an effective way to analyze network deployment as a whole. PLR must be closer to 0 for optimal network deployment, \ie, the minimum number of collisions and losses. We compute PLR as the ratio between the number of lost packets to the total number of sent packets. APD corresponds to the ratio between the sum of Packet Delays (PD) that were successfully received over the number of Total Received Packets ($TP_{Rx}$), as shown in Equation \ref{eq:apd}. PD means taking a packet from the source to its destination, adding the propagation and waiting time.

\begin{equation}
    \label{eq:apd}
    APD =  \frac{\sum_{u=1}^{U} PD_u}{TP_{Rx}} 
\end{equation}

%\blue{We repeated the experiments 33 times, and these repetitions presented statistically significant values, as we reached a 95\% confidence interval in the measurement of all tests performed. 
\green{We sent 1000 packets for each experiment, as indicated in Table \ref{tab:experiemtns}, and repeated the experiments 33 times. These repetitions presented statistically significant values, as we reached a 95\% confidence level in measuring all tests performed.} 
\brown{For instance, we calculate the confidence level using the standard error of the mean and the standard deviation of the sampling distribution of the mean. Equation \ref{eq:standard1} for the standard error of the mean of packets sent is}

\begin{equation}
\brown{    \label{eq:standard1}
    \sigma_m =  \frac{\sigma}{\sqrt{N}} }
\end{equation}

\hspace{-0.75cm}\brown{where $\sigma$ is the standard deviation and N is the sample size. When we calculate in a sample, the estimate of the standard error of the mean is shown in Equation \ref{eq:standard2}.}

\begin{equation}
\brown{    \label{eq:standard2}
    S_m =  \frac{S}{\sqrt{N}} }
\end{equation}

%\brown{We calculate the confidence level for this analysis using the probability density function for a normal continuous random variable, as presented in Equation \ref{eq:standard}.}

%\begin{equation}
%\brown{    \label{eq:standard}
%    f(x) =  \frac{exp(-x^2/2)}{\sqrt{2\pi}} }
%\end{equation}

%\hspace{-0.75cm} \brown{for a real number x. The probability density is defined in the standardized form.}
%We used the Statistical functions module (\textit{scipy.stats})\footnote{\scriptsize{https://docs.scipy.org/doc/scipy/reference/generated/scipy.stats.norm.html\#scipy.stats.norm}} to calculate the confidence level for this analysis.}
\blue{In our tests, the results show a consistent behavior both in simulation and in hardware tests.} Finally, we discuss the Multi-LoRa prototype results considering the experiments on a small-scale (testbed) and a large-scale (\blue{simulation}) analysis in the following subsections.


\subsection{Small-scale analysis}



Figure \ref{fig:delayTestbed} shows the delay for transmitting packets with different sizes considering three \sigla{} setups in the testbed environment. The delay results show that APD increases as soon as the packet size increases for transmitting data over Setup 1. Moreover, multi-radio architecture, \ie, Setup 2 and Setup 3 of \sigla{}, increases the APD lower than single-radio architecture for larger packet sizes. The weak performance of single-radio architecture is due to the half-duplex nature of the LoRa radio, where the queuing time on each hop is higher. For instance, packets with 256 bytes have APD 495\% higher than the packet size of 32 bytes by transmitting the packet over Setup 1. We divide each data packet into two small packets to transmit over each radio on Setup 2 and Setup 3, reducing the transmission time. Finally, it is possible to conclude that Setup 3 provides lower APD regardless of the packet size compared to the other architectures. It considers packet transmission over multiple radios to mitigate the half-duplex nature of the LoRa radio, and the BW value of 250 kHz helps to reduce APD.



%\lrp{%Nesse gráfico temos o resultado da medição de delay medio para pacotes de diferentes tamanhos. Mais uma  vez no ccenário Diop Pahm  existe um aumento quase que linear no delay médio dos pacotes.
%No setup1 e Setup 2 esse aumento de delay não é linear,  para os pacotes menores, os pacotes menore (16headr+8data  e 16head+16data) não são tão privilegidos com a divisão do pacotes em 2 radios devido ao head ser de 16 bytes,  que é maior que o dado em si. Já os pacotes de tamanho maior 128 e 256 tem um resultado melhor na redução do  delay médio  deviso a uma redução mais significativa  (pacote de 128 bytes vira  2x (16head + 56dados)  e 256bytes vira 2x(16head+120data) nesses casos comparados com o caso base existe uma redução significatva do delay. }

%\begin{figure}[!h]
%    \centering
%    \includegraphics[width=0.75\textwidth]{figures/apd_small.pdf}
%    \caption{APD for different packet size}
%    \label{fig:delayTestbed}
%\end{figure}

Figure \ref{fig:deliveyTestbed} shows the packet loss by transmitting \brown{different-sized packets} considering the three \sigla{} setups defined in the testbed environment. \brown{Analyzing the results makes} it is possible to conclude that the packet loss increases by around 2.1\% as soon as the packet size increases for transmitting data packets over Setup 1. %, since \dlr{pq? pacotes maiores tem mais tempo de transmissão e consequentemente maior probabilidade de colisão, erros de CRC, etc.}. 
However, Setup 2 and Setup 3 of \sigla{} increase the packet loss by around 1.3\%  for sending packets with the size of 64 bytes compared to the size of 32 bytes. % since \dlr{pq? Quando o pacote e maior que 64 bytes o tempo de processamento do pacote no nó acaba não aumentando as colisões de forma linear, pois }. 
Finally, Setup 3 has a packet loss of 1.1\% and 0.8\% lower than Setup 1 and Setup 2 for packet sizes ranging from 64 to 256. This performance of Setup 3 is due to the multi-radio characteristics compared to Setup 1 \brown{and} the SF and BW values compared to Setup 2, which reduces the collision probability in a multi-hop scenario.



%\dlr{Legal, mas pq esses comportamentos aconteceram? Principalmente esse crescimento inicial e cruzado. As justificativas estão nos comentários. Devemos usar?} 


%\dlr{um dado é dividido entre 2 radios (ou seja, metade do pacote é enviado em cada rádio). O pacote só é considerado como recebido caso chege nos 2 radios. Dependendo da aplicação o pacote pode ser retransmitido. No caso desse teste, o dado é restransmitido.}

%\sigla{} - Setup 2 provides the better data delivery compared to Diop and Pham and \sigla{} - Setup 1 architectures regardless the packet size. Specifically, \sigla{} - Setup 2 provides Loss \dlr{x\% and y\%} higher than Diop and Pham and \sigla{} - Setup 1, respectively. This is because \sigla{} - Setup 2 \dlr{explain}.

%\lrp{%Nesse gráfico onde temos  a taxa de perdas  médias para cada tamanho de pacote, pode-se  observar o comportamento do caso Diop an Pham  como sendo um comportamento base onde a medida que o tamanho dos pacotes aumentam a taxa de perda (geralmente devido a colisões) também aumenta  quase que de maneira  uniforme.
%No setup 1 e 2 pode-se observer um aumento da perda de pacotes maior quando comparamos os pacotes de 32 e 64 bytes, isso é devido a divisão do pacote em dois rádios (32 bytes- 2pacotes de (16head+8data)  e 64 bytes 2 pacotes (16head+16data) o que diminui o tamanho do pacote e consequentemente o time-to-air reduzindo assim as colisões. Já para os pacotes de 128 (2x16head+56data) e 256 bytes(2x 16head+120data) essa redução não não gera um impacto significativo nas colisões se comparados esses dois tamanhos de pacotes.Mas pode-se observar uma redução das colisões se comparado ao caso de Diop and Pham.}

%\begin{figure}[!h]
%    \centering
%    \includegraphics[width=0.75\textwidth]{figures/pdr_small.pdf}
%    \caption{Loss for different packet size}
%    \label{fig:deliveyTestbed}
%\end{figure}

\begin{figure}[!ht]
	\centering
	\subfigure[APD for different packet size]{
		\includegraphics[width=0.47\linewidth]{figures/apd_small.pdf}
		\label{fig:delayTestbed}
	}
	\subfigure[Loss for different packet size]{
		\includegraphics[width=0.47\linewidth]{figures/pdr_small.pdf}
		\label{fig:deliveyTestbed}
	}
	\caption{Testbed Results.}
	\label{fig:tesbed}
\end{figure}

\subsection{Large-scale analysis}



%\lrp{%Nessa ultima análise levantou-se o delay médio para um tamanho de pacote de 128bytes  entregando mensagens a nós que  estavam a até 6 saltos. com a mesma configuração da análise anterior. Neste cenário nem todos os nós participam ativamente da comunicação, todos os nós geram trafego de  sinalização (hello e routing packet)  e a comunicação é feita entre dois nós  com no máximo 6 saltos.
%O delay médio nos3 cenários tem um comportamento muito parecido, a medida que se adicionam mais nós na rede, aumentam os atrasos inseridos nos encaminhamentos o que pode ser percebido claramente entre 40 e 50 nós.
%O o cenário de Diop e o setup 1  para redes menores não paresetam diferenças significativas, porém para  redes maiores existe uma leve diminuição da inclinação da reta em relação  ao cenário de Diop.
%Já o setup 2 (devido a diminuição em quase 4x o delay médio da comunicação (2x pela divisão do pacote e 2 x pelo aumento da largura de banda 250MHz)  apresenta uma melhora significativa nos delays principalmente pela diminução do time-to-ais dos pacotes.}

Figure \ref{fig:delayEmulation} shows APD for several IoT nodes considering three \sigla{} setups in the \blue{simulation} environment. The APD results for the large scale-scenario show that Setup 3 provides APD 61.5\% and 26\% lower than Setup 1 and Setup 2. This behavior happens because Setup 3 considers a multi-radio transmission with a better radio configuration (\ie, BW and SF values). For instance, the packet with a payload of 128 bytes transmitted with SF 7 and BW of 125 kHz has a ToA value of 332.03 ms, while SF 7 and BW of 250 kHz has a ToA average value of 166.02 ms. This result explains the reason for the APD performance of \sigla{} - Setup 3 is 50\% better than Setup 2. Finally, Setup 2 provides APD results 75\% better than Setup 1 since Setup 2 considers two LoRa radios for transmitting data, reducing the effects of a half-duplex nature of the LoRa radio.

%\dlr{mais informação para completar a frase. Por exemplo, por que aumentou quase 600ms?}.

%\begin{figure}[!h]
%    \centering
%    \includegraphics[width=0.75\textwidth]{figures/apd_large.pdf}
%    \caption{APD for different number of nodes}
%    \label{fig:delayEmulation}
%\end{figure}


%\lrp{ Neste cenário nem todos os nós participam ativamente da comunicação, todos os nós geram trafego de  sinalização (hello e routing packet)  e a comunicação é feita entre dois nós  com no máximo 6 saltos.
%A perda média de pacotes no 3 cenários tem um comportamento muito parecido, a medida que se adicionam mais nós na rede, aumentam as colisões o que pode ser percevido claramente entre 30 e 50 nós.
%As perdas para o cenário de Diop e o setup 1  para redes menores não paresetam diferenças significativas, porém para  redes maiores existe uma diminuição em relação ao cenário de Diop.
%Já o setup 2 (devido a diminuição em quase 4x o delay médio da comunicação (2x pela divisão do pacote e 2 x pelo aumento da largura de banda 250MHz)  apresenta uma melhora significativa nas colisões, o principal causador das perdas}

Figure \ref{fig:deliveyEmulation} shows the PLR results in the \blue{simulation} environment considering deploying a different number of IoT nodes transmitting packets regarding the three \sigla{} setups. By analyzing the large-scale PLR results, we can conclude that PLR increases as soon as we increase the IoT nodes. PLR increases by around 2.9\% for Setup 3, conceding 10 IoT nodes compared to the deployment of 200 IoT nodes. This conceding is because more nodes increase the probability of collisions, especially in a multi-hop transmission.
In summary, Setup 3 provides the PLR of 1.02\% and 5.5\% compared to Setups 1 and 2, respectively, despite the number of IoT nodes. This behavior is due to its multi-radio transmission with a better LoRa radio configuration. The packet transmission with a higher BW value reduces ToA, where high ToA utilizes the wireless channel longer, increasing the collision probability \cite{moraes2020efficient}.


%\begin{figure}[!h]
%    \centering
%    \includegraphics[width=0.75\textwidth]{figures/pdr_large.pdf}
%    \caption{Loss for different number of nodes}
%    \label{fig:deliveyEmulation}
%\end{figure}

\begin{figure}[!ht]
	\centering
	\subfigure[APD for different number of nodes]{
		\includegraphics[width=0.47\linewidth]{figures/apd_large.pdf}
		\label{fig:delayEmulation}
	}
	\subfigure[Loss for different number of nodes]{
		\includegraphics[width=0.47\linewidth]{figures/pdr_large.pdf}
		\label{fig:deliveyEmulation}
	}
	\caption{Simulation Results}
	\label{fig:simulation}
\end{figure}


\subsection{\blue{Evaluation Conclusions}}

%\dlr{Acho que precisa uma conclusão/fechamento da seção, por exemplo linkando os resultados com o agro e nossa arquitetura/protótipo}
\blue{We conducted small-scale (testbed) and large-scale (simulation) experiments considering three \sigla{} setups to evaluate the impact of the multi-radio and different LoRa radio configurations. Our performance evaluation analysis identified that \sigla{} - Setup 3 has the best overall performance \brown{than} \sigla{} - Setup 1 and Setup 2 in both testbed and simulation scenarios. Setup 3 considers a multi-radio and multi-hop LoRa communication architecture with a better LoRa radio configuration. The multi-hop characteristic increases the coverage area for a large-scale IoT deployment, while the multi-radio mitigates the half-duplex nature of LoRa radio. However, \sigla{} - Setup 2 has a regular APD and PLR performance, associated with multi-radio characteristics without an exemplary LoRa radio configuration. \sigla{} - Setup 2 has limited results correlated with single-radio factors without a typical LoRa radio configuration.}



%\subsubsection{Methodology}

%We conducted the experiments in the \dlr{2nd floor of the Computer Engineering Department} at the UNISINOS. We deployed 8 IoT nodes (\ie, hardware prototype described in Section \ref{sec:Prototype}) in a grid topology of 3 $\times$ 3 and a LoRa Gateway on the edge. We consider the distance of 4m between each IoT node node in such grid topology. It is important to highlight the we reduced the radio range to \dlr{xm}, by \dlr{what}. In this sense, we can validate our hardware prototype in a controllable environment with a short size of 8 $\times$ 12 meters. Based on the such topology and radio configuration, each IoT nodes (\ie, source node) transmits data to LoRa Gateway (\ie, destination) over 1 to 3 hops between. 

%Each IoT node sends a data packet to the LoRa Gateway, and waits for an acknowledgment to send another data packet. At the end, each IoT node send 1.000 of data packet, since our goal is to evaluate the data deliver over a congested scenario. We define a set of four packet size for the data packets, \ie, 32, 64, 128, and 256 bytes, where the packet header has 16 bytes, as expected for many rural applications that sends data packet with different size. Table \ref{tab:experiemtns} summarizes the main experimental parameters.

%We repeated the experiments 33 times, and results show the values with a confidence interval of 95\%. We conducted experiments with the following setups, namely, \textit{based on Diop and Pham}, \textit{Multi-LoRa - Setup 1}, and \textit{Multi-LoRa - Setup 2}. Specifically,  \textit{based on Diop and Pham} means an multi-hop architecture with one radio configured with Spread Factor (SF) 7 and Bandwidth (BW) 125. On the other hand,  \textit{Multi-LoRa - Setup 1} means a multi-hop architecture with tow radio configured with SF 7 and BW 125. \dlr{pq escolhemos esses valores de SF e BW?} Finally, \textit{Multi-LoRa - Setup 2} means a multi-hop architecture with tow radio configured with SF 7 and BW 250. \dlr{pq escolhemos esses valores de SF e BW?}

%We used the following two performance metrics to evaluate the performance of the each setup, namely PDR and Average Packet Delay (APD). PDR $\in$ [0, 1] is an effective way to analyze the network deployment as a whole, \ie, in an optimal network deployment with a minimum number of collisions and losses, the value is close to 1. PDR is computed from the total number of received packets and the total number of transmitted packets over the network. On the other hand, APD corresponds to the ratio between the sum of Packet Delays (PD) that were successfully received over the number of Total Received Packets (TPRx), as Eq. \ref{eq:apd} shows. PD means the time taken for a packet from source to its destination, adding the propagation and waiting time.

%\begin{equation}
%    \label{eq:apd}
%    APD =  \frac{\sum_{u=1}^{U} PD_u}{TP_{Rx}} 
%\end{equation}

%\subsubsection{Results}


%\begin{figure}[!htb]
%    \centering
%    \includegraphics[width=0.6\textwidth]{figures/hwxsim}
%    \caption{Prototype x Simulator comparation}
%    \label{fig:simxhw}
%\end{figure}


%\subsubsection{Methodology}


%We conducted emulation experiments to evaluate the \sigla{} in terms of PDR and APD in a large-scale scenario, \ie, area of \dlr{100 km x 100 km} composed of 10 to 100 IoT nodes. The emulation is important to evaluate the scalability of \sigla{}, due to limited available IoT nodes in the testbed. We implemented the \sigla{} protocol stack \dlr{em qual linguagem? ou foi em cima de alguma ferrametna conhecida?}, where the emulation results has a similar behavior compared to testbed results, as Prade \et \cite{prade2020lora} shows. The simulation considers the \dlr{qual} path loss model, which is considered suitable for rural dta communication scenarios


%\dlr{We defined two scenario for emulation experiments in order to evaluate the performance of \sigla{} under different packet size transmission and number of IoT nodes.} In the Scenario 1, we deployed 20 IoT nodes in a grid topology with the distance of 4km between each IoT node node, and a LoRa Gateway on the edge. 
%Based on the such topology, each IoT nodes (\ie, source node) transmits data to LoRa Gateway (\ie, destination) over 1 to 6 hops between. For Scenario 2, we deployed 10 to 100 IoT nodes in a grid topology with the distance of 4km between each IoT node node, and a LoRa Gateway on the edge. 
%Based on the such topology, \dlr{each IoT nodes (\ie, source node) transmits data to LoRa Gateway (\ie, destination) over 1 to 6 hops between. }

%For both scenario, each IoT node sends a data packet to the LoRa Gateway, and waits for an acknowledgment to send another data packet. At the end, each IoT node send 1.000 of data packet, since our goal is to evaluate the data deliver over a congested scenario. For scenario 1, we define a set of four packet size for the data packets, \ie, 32, 64, 128, and 256 bytes. For scenario 2, each packet has the size of 128 bytes. Table \ref{tab:experiemtns} summarizes the main emulation parameters for both scenarios.


%We repeated the emulation experiments 33 times, and results show the values with a confidence interval of 95\%. We conducted experiments with the following setup, namely, \textit{based on Diop and Pham}, \textit{Multi-LoRa - Setup 1}, and \textit{Multi-LoRa - Setup 2}. We consider DR and APD to evaluate the performance of the each setup.


%\subsubsection{Results for different number of hops and packet size}


%\begin{figure}[!htb]
%    \centering
%    \subfigure[32 bytes]{
%        \includegraphics[width=0.45\textwidth]{figures/delay1.png}
%        \label{fig:delay1}
%    }
%    \subfigure[64 bytes]{
%        \includegraphics[width=0.45\textwidth]{figures/delay1.png}
%        \label{fig:delay2}
%    }
%    \subfigure[128 bytes]{
%        \includegraphics[width=0.45\textwidth]{figures/delay1.png}
%        \label{fig:delay3}
%    }
%    \subfigure[256 bytes]{
%        \includegraphics[width=0.45\textwidth]{figures/delay1.png}
%        \label{fig:delay4}
%    }
%    \caption{PLR on Different Number of Hops}
%    \label{fig:results1}
%\end{figure}

%\begin{figure}[!htb]
%    \centering
%    \subfigure[32 bytes]{
%        \includegraphics[width=0.45\textwidth]{figures/delay1.png}
%        \label{fig:delay1}
%    }
%    \subfigure[64 bytes]{
%        \includegraphics[width=0.45\textwidth]{figures/delay1.png}
%        \label{fig:delay2}
%    }
%    \subfigure[128 bytes]{
%        \includegraphics[width=0.45\textwidth]{figures/delay1.png}
%        \label{fig:delay3}
%    }
%    \subfigure[256 bytes]{
%        \includegraphics[width=0.45\textwidth]{figures/delay1.png}
%        \label{fig:delay4}
%    }
%    \caption{Delay on Different Number of Hops}
%    \label{fig:results2}
%\end{figure}


%\subsubsection{Results for different number of nodes}



%\begin{table}[!htb]
%    \centering
%    \caption{Parameters of evaluation for the \sigla{} architecture}
    %\scriptsize 
%    \footnotesize
%    \begin{tabular}{l|c|c|c}
%        \hline
%           &  & \multicolumn{2}{c}{Large-scale (emulation)} \\ \cline{3-4}
%        \multirow{-2}{*}{Characteristics}   & \multirow{-2}{*}{Small-scale (testbed)} & Scenario 1 &  Scenario 2  \\ \hline
        
        %% o que é diferente
        
%        \rowcolor{gray!10} Number of nodes & 8 & 20 & 10-100 \\
        
%        Field size & 8 x 12 (m) & 12 x 21 (km) & \dlr{?} \\
        
%        \rowcolor{gray!10} Topology & equidistant 4m  & \multicolumn{2}{c}{equidistant 4km} \\
        
%        Number of hops & 1-3 & 1-6 & 1-3 \\
        
%        \rowcolor{gray!10} Packet size (bytes)  & 32, 64, 128, 256 & 32, 64, 128, 256 & 128      \\ 
        

        %% o que é comum
         
%        Number of Packets (bytes)  & \multicolumn{3}{c}{1000}      \\
         
%        \rowcolor{gray!10} & \multicolumn{3}{c}{Diop and Pham \cite{mamour2019increased} (one radio with SF7 / 125 KHz)}      \\
%        \rowcolor{gray!10} Multi-LoRa configuration  & \multicolumn{3}{c}{Setup 1 (two radios with SF7 / 125 KHz)}      \\
%        \rowcolor{gray!10} & \multicolumn{3}{c}{Setup 2 (two radios with SF7 / 250 KHz)}   \\  \hline
%    \end{tabular}
%    \label{tab:experiemtns}
%\end{table}


==> old/sections_old/introduction.tex <==
\section{Introduction}

%apresentar smart farm e aplicaçõe semelhantes. Importância de monitoramento para essas aplicações e que não tem como colocar infra.

% ler aritog: https://www.mdpi.com/1424-8220/20/15/4273
% https://www.mdpi.com/1424-8220/20/13/3632
%http://www.libelium.com/resources/top_50_iot_sensor_applications_ranking/

%\blue{25 pages}% and 25 references!!}
The recent explosion of the Internet of things (IoT) technology \brown{dramatically changes} society through disruptive technologies in new sets of verticals and applications.
Smart farms/agriculture and rural electrical power distribution for the smart grid are a few examples of intelligent environment IoT verticals \cite{kulatunga2017opportunistic, visconti2020development}. 
In this context, IoT plays vital importance in supporting farmers in response to the global food challenge of feeding more than nine billion people in 2050 and the sustainability and competitiveness challenges. IoT devices could be deployed over huge areas in the farmlands to detect and collect soil information, precise climate, animal tracking, and information referred to growth or diseases of the cultivated crops \cite{visconti2020development}.
For example, there are farms with thousands of hectares for cotton planting\brown{, in Brazil.} In this case, cotton packages are left on the farm for long periods, and they can catch fire with humidity below 12\%. Therefore, monitoring the farmland avoids financial losses and extensive burning to increase agriculture efficiency in continental countries with an agricultural vocation.

IoT technologies help to produce high-quality fruits and vegetables in sufficient quantities to satisfy food requirements while maintaining competitive costs \cite{visconti2020development}. The collected data must feed decision-support systems to provide precision dairy farming information, and thus plants and animals get precisely the treatment they need in a data-driven fashion. The improvements in productivity and environmental sustainability rely on the analytics' accuracy, which strongly depends on the amount and timeliness of the data collected \cite{kulatunga2017opportunistic}. Therefore, it is essential to provide data acquisition in farms where network connectivity is a constraint. The data acquisition solution must ensure timely, efficient, and reliable communication and performance longevity for IoT devices deployed over huge farmlands \cite{kulatunga2017opportunistic}. 

Innovative long-range technologies, such as Long-Range Wide Area Network (LoRaWAN), attract attention from both academia and industry to capture long-range communication requirements through promising capabilities in a broad area \brown{of} unlicensed frequency bands with low power consumption and low throughput \cite{dantas2021Survey}. %In this context, the Long-Range Wide Area Network (LoRaWAN) architecture is considered the most adopted LPWAN architecture for its ubiquitous connectivity capacities in outdoor use cases \cite{matni2020experimenting}. 
%\dlr{In particular, LoRa physical layer is a proprietary spread spectrum modulation based on the robust Chirp Spread Spectrum (CSS) by Semtech \cite{lyu2019achieving}. Based on the LoRa physical layer, the LoRa Alliance \cite{alliance2015white} defined the higher layers and network architecture of the Long-Range Wide Area Network (LoRaWAN) \cite{croce2018impact}.}
LoRaWAN architecture considers a single-hop communication between the IoT device and gateway over several channels, forming a star network topology. %IoT devices broadcast messages for neighbor gateways, which forwards the message to the application server through an existing IP network. 
Based on such architecture, LoRaWAN provides connectivity to IoT devices deployed over a vast area by employing a control access mechanism with less complexity at low throughput \cite{qadir2018low}. Specifically, LoRaWAN achieves a nearly 2-5 km coverage range in urban areas and about 45 km in rural areas \cite{8783184}. Therefore, the low-power, low-cost, and long-range properties provided by LoRaWAN allow devices to spread and move over large geographic areas \cite{dantas2021Survey}. 

% J. M. Marais, R. Malekian and A. M. Abu-Mahfouz, "Evaluating the LoRaWAN Protocol Using a Permanent Outdoor Testbed," in IEEE Sensors Journal, vol. 19, no. 12, pp. 4726-4733, 15 June15, 2019, doi: 10.1109/JSEN.2019.2900735. Esse trabalho pode ser usado para citar uma cobertura menor da rede lorawan (práticamente 5 km de raio e não os 45 teóricos)

\brown{Even though LoRaWAN provides broad coverage in rural areas with a gateway, it might not be sufficient for data acquisition on farms of hundreds of square kilometers \cite{Huang-Chen}.} The deployment of more gateways could be integrated into the network ecosystems to increase the coverage area. However, deploying gateways leads to high Capital Expenditure (CAPEX) and Operational Expenditure (OPEX), including the cost of a gateway, leasing, maintenance, etc. \cite{dantas2021Survey}. Therefore, a multi-hop network \brown{is essential} in applications requiring extensive deployment, which is not addressed by LoRaWAN architecture \cite{cotrim2020lorawan, dantas2021Survey}. Specifically, it is possible to consider multi-hop communication among the gateways, IoT devices, or both to increase the coverage area \cite{cotrim2020lorawan}. Nevertheless, it is not convenient or feasible to deploy multiple gateways in a farm scenario, mainly due to costs. However, IoT devices could monitor the environment and work as a relay with reduced cost to provide connectivity for any IoT device deployed over large areas in the farmlands \cite{kulatunga2017opportunistic}. \blue{Therefore, it is fundamental to design a multi-hop architecture by considering only a hop on the LoRaWAN radio, a.k.a., LoRa radio.} 

\green{Besides the benefits of multi-hop communication, multiple radios mitigate the collision caused by the half-duplex nature of LoRa radio. For instance, various radios decrease the use of the channel to send a packet, which reduces the collision rate. However, higher layers (MAC and routing layers) must consider an efficient transmission scheme over multiple radios. For instance, the MAC layer must efficiently manage the access control layer of multiple radios. In contrast, the routing layer must meet the characteristics of this multi-hop and multi-radio architecture, such as lower signaling overhead and use of half-duplex communication. Moreover, higher layers must consider the key application requirements individually rather than a one-fits-all solution to best serve the limited resources of such multi-hop and multi-radio architecture. Therefore, it is fundamental to design an efficient multi-hop and multi-radio architecture to transmit data with different regiments of IoT devices deployed over large-scale rural IoT scenarios, which is still an open issue. However, to the best of our knowledge, the state-of-the-art does not present an architecture that integrates multi-hop, multi-radio LoRa communication, and service requirements awareness for each application in an efficient solution for large-scale rural IoT scenarios.}




%pergunta de pesquisa: como transmitir serviços com maior alcance e diferentes requisitos de atraso e vazão para aplicações IoT em ambientes rurais?

%\dlr{This scenario leads to the need to design an efficient architecture to enable multi-hop communication for large scale IoT deployment in rural areas.} Arquitetura com pouca complexidade e baixo custo.


Based on this challenge in mind, we propose a multi-radio and multi-hop LoRa communication architecture to increase the coverage and service for large-scale IoT deployment in rural areas, called \sigla{}. It provides a reference for \brown{implementing} communication networks based on the physical layer LoRa. The \sigla{} architecture considers an ad hoc network topology to increase the coverage area. Moreover, we design data multiplexing mechanisms in multiple LoRa radios to increase throughput and reduce collisions. Furthermore, the architecture prioritizes specific data types, decreasing the jitter among the hops of the network. Finally, we introduce an experimental case study to analyze the performance of the proposed architecture. The main contributions are summarized: 
\begin{inparaenum}[($i)$]
    \item We present a \sigla{} architecture to enable multi-radio and multi-hop LoRa communication between IoT devices running applications with monitoring service requirements.
    \brown{\item We introduce a hardware prototype for physically implementing the Multi-LoRa architecture, which consists of implementation in both hardware and software.}
    %\item We introduce a hardware prototype for physically implementing the \sigla{} architecture consists of hardware and software implementation.
    \brown{\item A simulation environment based on the same software in the hardware prototype to support scalability analyses.}
    \item We perform real experiments to introduce the impacts and benefits of \sigla{}. The results show that \sigla{} can effectively mitigate the challenges of multi-hop communication over LoRa for large-scale IoT deployment in rural areas to increase connectivity.
\end{inparaenum}    



This article extends the previous work described in Prade et al. \cite{prade2020lora}. Its main contributions include an extensive review of the state-of-the-art, a more detailed description of the \sigla{} architecture, and a comprehensive performance evaluation of \sigla{} in rural areas to increase connectivity. The article is organized as follows. Section~\ref{sec:relatedworks} introduces the related work about multi-hop LoRa communication. Section~\ref{sec:prop} presents \sigla{} for improving the coverage of LoRa communication in large-scale IoT scenarios. Section \ref{sec:Prototype} describes prototype implementation, and Section~\ref{sec:metrics} introduces an experimental case study to analyze the performance of the proposed architecture. Finally, Section~\ref{sec:conc} concludes the work and \brown{presents} the future work.


==> old/sections_old/relatedwork.tex <==
\section{Related Work}
\label{sec:relatedworks}


This section presents the state-of-the-art, which focuses on multi-radio and multi-hop communication for LoRa radios. In each work, we discuss \brown{its} advantages and disadvantages.
%% Multi-radio
A group of works focused on multi-radio approaches. Mikhaylov et al. \cite{mikhaylov2018multi} looked into the feasibility of creating a multi-RAT Low Power Wide Area Network (LPWAN) system that could fulfill transmission requirements in a scenario where Narrow Band IoT (NB-IoT) and Long Term Evolution (LTE) coexisted. The authors built a device prototype \brown{with} an NB-IoT chipset that handles communication events and implements the Lo-RaWAN module. Moreover, the authors tested the dual-RAT LPWAN device in a commercial NB-IoT and a private LoRaWAN environment at the Brno University of Technology in the Czech Republic. According to the findings, the NB-IoT chipset consumed more than 200 mW on average to maintain network synchronization. However, the LoRaWAN transceiver \brown{used} less than 60 mW due to the lower transmission power, despite the longer transmission time.

\green{Huang-Chen and Kai-Hsiang \cite{Huang-Chen} proposed a LoRa mesh networking system for collecting data from IoT sensors deployed over a large geographical area. Moreover, the authors analyzed the communication performance of the proposed LoRa mesh network, where the obtained result shows that the LoRa mesh network archived better delivery performance. The LoRa mesh network module can be integrated with other IoT applications to collect data from distributed sensors, bypassing complex data transmission and collection issues. Users do not need to know how to build a network to route the data because the communication protocols are contained in the module. This solution significantly simplifies long-range wireless communication and facilitates IoT applications over large regions.}

Kim et al. \cite{kim2016low} implemented a multi-interface IoT System device based on Wi-Fi and LoRa using a sensor data system. The multi-interface device collects data from each sensor and redirects it to one of two handlers: (\textit{i}) the Wi-Fi handler carries the wireless packet via Wi-Fi, and (\textit{ii}) the LoRaWAN handler sends the sensor data via the LoRaWAN module network. The multi-interface device selects the best approach (Wi-Fi or LoRaWAN) to transmit the packet based on the data type using a power and data scheduler. The authors assessed the performance by deploying a real-world infrastructure scenario at the beach (wireless LAN AP, station, and LoRaWAN gateway). The numerical results show that as the distance increases, the RSSI value and data rate decrease, demonstrating the sensitivity of the Wi-Fi card. The RSSI results are similar in both antennas at any distance, and the higher the antenna gain, the higher the SNR value.

\blue{Queralta et al. \cite{queralta2019edge} planned a framework engineering for managing IoT-based medical services frameworks, especially electrocardiography checking frameworks that need to play out the information \brown{preparation} and pressure at the edge of the organization. The authors consolidated edge and mist processing ideas with LoRaWAN and profound learning predictions to construct a five-layer framework, particularly sensor, edge, fog, cloud, and application. The authors directed their trials in a metropolitan climate in Turku, Finland, to evaluate the achievability of the design. The assessment results show that occasion distinguishing proof happens with an average level of exactness of more than 90\% and a regular review of more than 95\% in fall detection through this engineering.} 
\brown{It decreases the computational heap of the sensor hubs via completing well-being checking tasks in edge passages.}
%It decreases the computational heap of the sensor hubs via completing well-being checking errands in edge-passages.}

%Queralta et al. \cite{queralta2019edge} planned a framework engineering for managing IoT-based medical services frameworks, especially electrocardiography checking frameworks that need to play out the information preparing and pressure at the organization edge. The authors consolidated edge and mist processing ideas with LoRaWAN and profound learning predictions for constructing a five-layer framework particularly sensor layer, edge layer, fog layer, cloud layer, and the application layer. \dlr{To approve the design's achievability, the authors directed their trials in a metropolitan climate in Turku, Finland.} The assessment results show that occasion distinguishing proof happens with an average level of exactness of more than 90\% and a regular review of more than 95\% in fall detection through this engineering. It additionally decreases the computational heap of the sensor hubs via completing well-being checking errands in edge-passages.

%%%% Multi-hop

The literature presents some strategies for multi-hop between gateways. Lundell \et~\cite{lundell2018routing} introduced a protocol based on Hybrid Wireless Mesh Protocol (HWMP) and Ad-hoc On-Demand Distance Vector Routing (AODV) to improve network communication and provide broad coverage. The routing protocol defines the operations of the gateways when it receives an uplink from an end device. Case root mode is used for routing, the gateway verifies a valid path to the root node, and if so, it transmits the packet. However, if no such way exists or root mode is not used, the gateway does route discovery. Otherwise, if the gateway is the destination with Internet connectivity, it decapsulates the data packet to obtain the original LoRaWAN message, transfers it to the network server, and awaits an answer. \brown{The routing method is transparent to end devices and the network server in this context.}
%In this context, the routing method is transparent to end devices and the network server.



Dwijaksara \et~\cite{dwijaksara2019multihop} presented a multi-hop LoRa gateway-to-gateway communication protocol that explicitly performs all three constraints (\textit{i.e.}, packet size, duty cycle, and time) required on LoRa networks. The proposed protocol introduces two functionalities of routing and channel access. The routing protocol encounters a route from an end device to the network server (\textit{i.e.}, a list of forwarding gateways). The channel access scheme designates the packet transmission mechanism within two gateway. Moreover, Multi-hop considering end devices have made progress in the last few years, \textit{e.g.}, Anneda \et~\cite{anedda2018energy} describe a solution called e2McH, performing energy-efficient communications in multi-hop LoRaWAN routing between the end devices. The algorithm aims to find the neighbor end device closer to the gateway and find the best path to transmit data to the network server.


Ebi \et~\cite{ebi2019synchronous} introduced a LoRaWAN architecture to mitigate the monitoring of underground infrastructure. The architecture comprises sensor devices building a LoRa mesh network posting data to a repeater device, operating as a sink for the sensors. The repeater device corresponds directly with the central gateway, and it may be a mere battery-powered end device that is not connected to the Internet. The repeater node works as a relay that delivers the data to the gateway, and the sensor devices serve as routers in the mesh network. The authors carried \brown{out} two department analyses as a proof-of-concept. Repeater and router devices are energy-constrained, single-channel (repeater with two radios), and execute a synchronization mechanism.


Dias \et~\cite{dias2020multi} developed a routing protocol that uses the LoRaWAN beacon to deliver packets from end devices to gateways through a minimum number of hops. The solution \brown{adapts} the Destination-Sequenced Distance Vector (DSDV) protocol, where the end device routers are static, and there is synchronization between nodes. Moreover, the end devices are classified into two varieties: the routing nodes and the leaf nodes, where the routing devices are non-energy constrained. Moreover, Sisinni \et~\cite{sisinni2019lorawan} validate and implement a proof-of-concept prototype of an enhanced LoRaWAN node (e-Node) in an industrial scenario to extend the coverage of messages transmitted using the highest data rates. The authors presented coverage tests to measure the signal strength to ensure the proper performance of the proposal and demonstrate its effectiveness in increasing the range. Finally, Diop \et~\cite{mamour2019increased} proposed a multi-hop solution to extend the LoRa network coverage in rural areas. The authors introduced a simplistic message forwarder and a synchronization method. Furthermore, the principal purpose is to produce an intelligent, transparent, and battery-operated intermediate node–relay device joined after a deployment campaign to seamlessly afford an extra hop between the separated devices and the gateway. 



%Loginov et al. \cite{loginov2018study} proposed an strategy to reduce the network latency in multi-hop LoRaWAN transmissions. Specifically, the strategy consists of instantly retry the first transmission attempt when first collision was detected, \ie, retry transmission without back off if. Inspired in the Transmission Opportunity (TXOP) sharing feature from the WiFi and adapting the p-persistent extension from slotted ALOHA, They develop an analytical model based on the Markov Chain.



%\textcolor{green}{Não editar esta seção [Lúcio]}

%Pegar os artigos desse Survey:
%LoRaWAN Mesh Networks: A Review and Classification of Multihop Communication

%\textcolor{blue}{Acho que dá para fazer um background bem focado sobre as três combinações de \textit{Multiple Gateway and Routing} definidas por Panicker J.G. (2019):} 

%\begin{itemize}
 %   \item \textbf{Rede de malha usando vários gateways LoRa}, onde vários roteadores LoRa gateway são configurados para aumentar a área de cobertura. Pelo menos um dos gateways deve ser considerado como o 'Root' e o (s) mesmo (s) gateway (s) terão conectividade ativa de rede, portanto, seria diretamente acessível polo usuário via internet / nuvem ou uma configuração local. Os outros gateways seria usado como repetidor de malha para aumentar a área de cobertura. Os gateways podem ser montados em pólos para obter links LOS, se o terreno permitir.
  %  \item \textbf{Rede Mesh usando nós LoRa}, uma alternativa seria formar uma rede de malha com os próprios nós emparelhados com um único gateway, foi projetado para compreender um único gateway, mas todo nó LoRa (cliente) atua como um gateway intermediário. Se o nó vai além da cobertura do gateway LoRa, os nós LoRa formam uma rede de malha e haverá um nó direto para o nó comunicação. O gateway enviaria sinais para mapear os gráficos, permitindo formação dinâmica de links únicos ou múltiplos, consequentemente, o sistema identificará as melhores caminho (s).
   % \item \textbf{Rede Mesh usando nós LoRa e múltiplos Roteadores de gateway LoRa}, este modelo é uma combinação do modelo A e do modelo B, neste mode existem vários gateways dos quais o nó raiz tenha uma conexão de rede ativa e o resto podem se espalhar estrategicamente, os nós são programados para suportar comunicação nó a nó conforme discutido no Modelo B, e os gateways são programados para suportar a comunicação de gateway para gateway, conforme discutido no Modelo A. No Modelo C, os roteadores de gateway não raiz atuam como repetidores de malha e atingem periodicamente a rota mapeada do gateway raiz e emprega o LoRaWAN como protocolo de roteamento.
%\end{itemize}


%podemos separar os trabalhos que são relay-gw e relay-node.

%Improving the Capacity of a Mesh LoRa Network by Spreading-Factor-Based Network Clustering

%An Adaptive Spreading Factor Selection Scheme for a Single Channel LoRa Modem

%LoRaWAN Mesh Networks: A Review and Classification of Multihop Communication




 %\textcolor{red}{Lúcio: precisamos deixar essa seção em +- 1 página: \\ 1) Como podemos agrupar esses trabalhos? (i) Roteamento, (ii) Controle de acesso, (iii) ambos/outros \\ 2) Quais são as colunas interessantes para fazer uma tabela comparativa desses trabalhos?}


\green{We focus on three main characteristics to analyze the state-of-the-art: 
\begin{inparaenum}[($i)$] 
    \item type of multi-hop communication,
    \item multi-radio communication, and
    \item service requirements awareness for each application.
\end{inparaenum} 
These characteristics together highlight the major contribution of this article compared to existing literature. In this way, Table \ref{tab:related_works} summarizes our state-of-the-art review of multi-hop and multi-radio for LoRa communication in large-scale scenarios. Based on our state-of-the-art analysis, we argue that no one work considers a multi-hop, multi-radio, and priority-aware transmission together. Some studies are considered multi-hop between either IoT devices or gateways \cite{Huang-Chen, lundell2018routing, dwijaksara2019multihop, anedda2018energy,ebi2019synchronous, dias2020multi,mamour2019increased, sisinni2019lorawan}. Moreover, as we can observe, few works \brown{are considered} multi-radio \cite{mikhaylov2018multi, kim2016low, queralta2019edge}. Requirement-based, \ie, analyzing application requirements, is only \brown{viewed by articles} \cite{ ebi2019synchronous, mamour2019increased, sisinni2019lorawan, queralta2019edge}, which is an essential issue for application requirements. To the best of our knowledge, only Multi-LoRa combines every critical feature previously mentioned not provided by existing multi-hop LoRa communication architectures in large-scale rural IoT scenarios.}

%MESH (acesso ao meio - multi-hop)   |   multi-radio (MIMO)  | Prioridade (escalonamento)

\begin{table*}[!h]
    \centering
    \caption{Analyzed studies about multi-hop and multi-radio in large-scale scenarios}
    \label{Tab:related}
    %\scriptsize 
    \footnotesize
    \begin{tabular}{l|c|c|c|c}
        \hline
        Work                     & Year & Multi-hop & Multi-radio  & Requirement-aware \\ \hline
        
        \rowcolor{gray!10} Queralta et al. \cite{queralta2019edge}  & 2019 &     -      &     Multi-radio         &        Medical       \\
        
        Mikhaylov et al.  \cite{mikhaylov2018multi}  & 2018 &  -       &    Multi-radio       &  -\\
        
         \rowcolor{gray!10} Kim  et  al.  \cite{kim2016low}  & 2016 &     -      &     Multi-radio  &        -        \\
        
        Lundell \et~\cite{lundell2018routing} & 2018 &  Gateways       &    -          &      -          \\
        
        \rowcolor{gray!10} Dwijaksara \et~\cite{dwijaksara2019multihop} & 2019 &  Gateways         &     -      &      -          \\
        
        Anneda \et~\cite{anedda2018energy} & 2018 &   IoT devices        &    -          &         -       \\
        
        \rowcolor{gray!10}  &  &  &     &          Underground   \\
        \rowcolor{gray!10} \multirow{-2}{*}{Ebi \et~\cite{ebi2019synchronous}}  & \multirow{-2}{*}{2019} & \multirow{-2}{*}{IoT devices}  &  \multirow{-2}{*}{ - }        &  infrastructure  \\
        
        Dias \et~\cite{dias2020multi} & 2020 &  IoT devices       &     -         &       -         \\
        
        \rowcolor{gray!10} Diop \et~\cite{mamour2019increased} & 2019 & IoT devices      &        -      &     Rural areas          \\
        
        Sisinni \et~\cite{sisinni2019lorawan}  & 2019 &  IoT devices        &     -         &    industrial       \\
 
        \rowcolor{gray!10} \green{Huang-Chen and} &  &  &     &    \\
        \rowcolor{gray!10} \green{Kai-Hsiang \cite{Huang-Chen}}  & \multirow{-2}{*}{\green{2018}} & \multirow{-2}{*}{\green{IoT devices}}  &  \multirow{-2}{*}{\green{-}}  &  \multirow{-2}{*}{\green{-}}   \\
        
        \rowcolor{blue!30} &  &   & Multiplexing  & Priority-aware  \\ 
        \rowcolor{blue!30} \multirow{-2}{*}{\textbf{\sigla{}} } & \multirow{-2}{*}{2021} & \multirow{-2}{*}{IoT devices} & mechanisms & transmission \\ \hline
    \end{tabular}
    \label{tab:related_works}
\end{table*}


%\dlr{highlight here WHY this design IS IMPORTANT, but not propose YET-ANOTHER LoRa Mesh}

%\dlr{precisamos adicionar \cite{Huang-Chen} nesse texto}




==> old/sections_old/relatedwork_old.tex <==
\section{Related Work}
\label{sec:relatedworks}

% Pensar se é necessário uma subseção apresentando o que é LoRa.


podemos separar os trabalhos que são relay-gw e relay-node.

Improving the Capacity of a Mesh LoRa Network by Spreading-Factor-Based Network Clustering

An Adaptive Spreading Factor Selection Scheme for a Single Channel LoRa Modem

LoRaWAN Mesh Networks: A Review and Classification of Multihop Communication

Loginov et al. \cite{loginov2018study} proposed an strategy to reduce the network latency in multi-hop LoRaWAN transmissions. Specifically, the strategy consists of instantly retry the first transmission attempt when first collision was detected, \ie, retry transmission without back off if. Inspired in the Transmission Opportunity (TXOP) sharing feature from the WiFi and adapting the p-persistent extension from slotted ALOHA, They develop an analytical model based on the Markov Chain.


 \textcolor{red}{Lúcio: precisamos deixar essa seção em +- 1 página: \\ 1) Como podemos agrupar esses trabalhos? (i) Roteamento, (ii) Controle de acesso, (iii) ambos/outros \\ 2) Quais são as colunas interessantes para fazer uma tabela comparativa desses trabalhos?}

% Lundell, Daniel, et al. "A routing protocol for LoRa mesh networks." 2018 IEEE 19th International Symposium on" A World of Wireless, Mobile and Multimedia Networks"(WoWMoM). IEEE, 2018
\textbf{Tag:Trabalho de roteamento} - Lundell D. \cite{Lundell-18} toma como ponto de partida o Hybrid Wireless Mesh Protocol (HWMP) como protocolo de roteamento LoRa para estruturar seu próprio protocolo LPWAN. O HWMP oferece baixo custo de ponta a ponta e atrasos no tráfego de dados pelo uso de roteamento proativo, enquanto ao mesmo tempo, sem exigir a inundação de topologia em toda a rede em formação. O autor enfatiza a remoção de recursos adicionais do protocolo no emprego do mesmo numa rede LoRa. O trabalho combinar assim o design geral do protocolo do HWMP com alguns aspectos emprestado do protocolo Ad-hoc On Demand Distance Vector (AODV) usando recursos de informações de cabeçalho mais simplificadas pertinentes a este. O protocolo funciona com princípio de tunelamento, o gateway recebe um pacote de um dispositivo final, se não possuir uma conexão com a Internet, ele encaminhará o pacote de duas maneiras possíveis. Se um nó raiz foi configurado na rede, aplica-se o modo pró-ativo do HWMP e o gateway encaminha o pacote para o nó de rota ao longo do rota já estabelecida. Se não houver nó raiz, o gateway procurará uma rota para um gateway conectado à Internet. Encaminhamento ocorre apenas entre gateways e é transparente para os dois dispositivos finais e o servidor de rede LoRa. As mensagens do protocolo de roteamento de AODV e HWMP precisa ser modificado para funcionar com o LoRaWAN. Gateways reconhecidos roteia os pacotes usando o cabeçalho LoRaWAN MAC, onde definimos o campo MType como 111, reservado no LoRaWAN especificação para formatos de mensagem não padrão. Usa-se o campo RFU, reservado para uso futuro, para 001 para identificar nosso protocolo de roteamento. O cabeçalho original é mantido para que o pacote pode ser reconhecido como um pacote LoRaWAN no rede. Para os Gateways dentro da rede usam seus 8 endereços MAC de byte, também chamados de ID do nó a seguir, para se identificarem, como os dispositivos finais não participam de roteamento, reduz-se a sobrecarga necessária usando o software de 4 bytes endereço do dispositivo para identificar os dispositivos finais. O protocolo opera seguindo as etapas: Primeiro, um dispositivo final acorda e transmite uma mensagem. Isso então aguarda a abertura de sua primeira janela de recebimento. O gateway é constantemente ouvindo e recebe a mensagem do final dispositivo. Se o modo raiz for usado para roteamento, o gateway então verifica se possui um caminho válido para o nó raiz e, se houver, encaminha o pacote. Se esse caminho não existir ou o modo raiz for não usado, o gateway executa a descoberta de rota.  \textcolor{blue}{Neste trabalho, o autor usa a estrutura de uma rede LoRAWAN e o protocolo LoRAWAN MAC como  base  para desenvolver uma rede mesh com os dispositivos finais, fazendo com que  a topologia estrela da rede LoRAWAN  seja ampliada com roteamento (saltos) mesh entre os (sensores). Ele empacote os protocolos de roteamento adaptados por ele dentro do pacote LoRAWAN, isso causa um overhead enorme,  visto que em alguns casos o pacote LORAWAN dispões de apenas 11 bytes de dados. No trabalho desenvolvido como ele não usa como base LoRAWA, esse overhead é  reduzido,  dos 256 bytes de dados permitidos na modulação LoRA,  apenas 16 são utilizados para enderereçemento e roteamento,  ficando disponível  240 bytes em cada pacote para dados. A  arquitetura desenvolvida também não necessita de gateways LoRAWA ( infra mais cara), é uma rede auto organizavel. Poré, pode apresentar um maior número de colsões de pacotes, se comparado ao lorawan, mas a solução de  multiplexar o pacote em 2 canais reduz o tepo de cada pacote, consequentemente reduzindo as colisões. }

% Zhu, Guibing, et al. "Improving the capacity of a mesh LoRa network by spreading-factor-based network clustering." IEEE Access 7 (2019): 21584-21596.
\textbf{Tag:Trabalho de melhoria da capacidade} - Zhu G. \cite{Zhu-19} enfatiza que os protocolos propostos para redes LoRa geralmente constroem uma abordagem de atribuição de canal estático para manter a simplicidade da coordenação do canal ou semelhante à alocação de SF em uma rede em malha LoRa, a adoção da transmissão paralela usando vários canais já foi implementado de forma conveniente redes internacionais de coleta de dados de raiz única multip hop. Como proposta para alcançar a melhoria da capacidade por transmissão paralela, seu trabalho têm como objetivo separar uma rede totalmente conectada em várias sub-redes desconexas com diferentes SFs. Especificamente, cada nó é alocado com um único SF e os nós usando o mesmo SF forma uma sub-rede multi-hop que opera independentemente com os outros. Portanto três aspectos relevantes são considerados para maximizar a capacidade da rede inteira. Primeiro, o tráfego precisa ser descarregado para cada sub-rede de maneira equilibrada para impedir que qualquer sub-rede se torne o gargalo da taxa de transferência; Segundo, cada sub-rede precisa estar bem conectado sem nós inacessíveis; Terceiro, com uma adequada alocação SF, o diâmetro de cada sub-rede também pode ser potencialmente reduzido para que a capacidade seja ainda melhorado. Para tanto enfatiza como o tree-based SF clustering algorithm (TSCA), algoritmo que gera a topologia de cada sub-rede, como proposta de alcança os três aspectos mencionados.
\textcolor{blue}{Neste trabalho, o propões  particionamento da rede usando diferentes SF, isso reduz  colisões melhorando esse quesito, porém trabalhando com  diferentes SF, o tempo  de envio de pacotes muda drasticamente, chegando a dobrar ou quadruplicar em algun casos. Hopes com diferetes SF tornam a rede menos deterministica e  com maior jitter. Como da da minha arquitetura   foi conseguir uma rede mais determinitica possível, não foi particionada por SF. Mas esse trabalho serviu como base para o estudo de particionamto da rede, determinando um nímero  ótimo de saltos (Figura 8 e 9). Mas a técnica de particionamento empregada foi o uso de diferentes canais (frequencia e sempre o mesmo SF  para manter o tempo de pacote em cada salto sempre igual) }

% https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8048465
\textbf{Tag:Trabalho de controle de acesso ao meio} - Chun-Hao Liao \cite{Liao-17}, para melhorar ainda mais a confiabilidade do receptor, o autor promove colocar o método de offset-CT, que é um método simples, mas eficaz para aumentar o deslocamento de tempo entre os pacotes enquanto mantém um alinhamento de tempo virtual de cada salto. A novidade desta proposta é dupla: primeiro, pela prática de uso da técnica CT-LoRa, onde o número do transmissor não pode ser determinado, o autor propõe introdução de um atraso de tempo aleatório distribuído uniformemente entre 0 e o tempo de um símbolo antes de toda retransmissão do pacote. Segundo, a fim de evitar que o desvio de tempo divergir, pretende realizar as informações de atraso em cada pacote, para nó desmodular com êxito o pacote poderia inserir o complemento atraso necessário para alinhar o tempo. Após observando que este método é somente viável para a tecnologia como LoRa que sobrevive ao CT (protocolo de inundação) puramente pelo efeito de captura. O autor testa dois cenários típicos, cenário de baixa densidade e o caso de alta densidade. O cenário típico vários resultados mostram que o CT-LoRa é muito confiável mesmo sem offset-CT. Em seguida, testa o cenário crítico para CT, onde vários nós próximos uns dos outros para tornar o deslocamento de energia entre o pacote muito pequeno. CT é um protocolo de rede na camada de link para redes sem fio multi-hop, em cada inundação de pacotes, haveria  apenas um nó servindo como iniciador. O iniciador transmitir o primeiro pacote para desencadear a inundação. Cada nó quem recebe o pacote com sucesso pela primeira vez e depois execute a retransmissão imediata como outra transmissão. O mesmo procedimento continua até que o pacote seja inundado toda a rede. A diferença essencial entre a CT e protocolo de camada de link convencional (por exemplo, CSMA / CA adotado em IEEE 802.15.4) é a visão para colisões de pacotes. Enquanto os convencionais se esforçam para evitar colisões de pacotes, O CT abraça as colisões sincronizadas de pacotes que acontecem quando vários nos executam retransmissões imediatas ao mesmo tempo. Removendo a sobrecarga da colisão, evita-se mecanismo de proteção, o pacote pode inundar a rede muito rapidamente através dos nos. Esta propriedade é particularmente importante ao construir uma rede multi-hop LoRa, já que os pacotes LoRa tendem a ser longos (uma ordem de milissegundos a segundos) e o convencional mecanismo de prevenção de colisão poderia resultar facilmente em muito longa latência e tempo de despertar.\textcolor{blue}{Neste trabalho, o autor busca um mecanismo eficaz para  o problema das colisões. Quanto maiores os pacotes LoRA, maior a probabilidade de colisões. A  minha arquitetura não implementa nenhum mecanismo de tratamento de colisões, ela deixa a cargo da camada de aplicação o retransmissão por timeout.  Poré, como os pacotes LoRa utilizados geralmente usam o tamanho máximo permitido na especificação (255 bytes) pode apresentar um maior número de colsões de pacotes. Nesse sentido  a solução de  multiplexar o pacote em 2 canais com frequencias diferentes e mesmo SF reduz o tepo de cada pacote, consequentemente reduzindo as colisões. }

% Sato, Goshi, Yoshitaka Shibata, and Noriki Uchida. "Study on Balloon Network Using LoRa Mesh Communication System." Workshops of the International Conference on Advanced Information Networking and Applications. Springer, Cham, 2019.
\textbf{Tag:Trabalho de controle de acesso ao meio} Sato G. \cite{Sato-19} avaliar os procedimentos e o tempo de construção da rede aérea, tempo de operação contínua e esclarecer a diferença de características de  comunicação no solo e comunicação aérea, vantagens e desvantagens, medir a taxa de transferência efetiva da rede construída e o tempo necessário para os dados sincronização e avaliar se ele atende aos requisitos do aplicativo a ser implementado. Como a comunicação sem fio LoRa usa comunicação de transmissão, se ocorre colisão de sinais sem fio devido à transmissão simultânea, a retransmissão é não realizado. Além disso, considerando vários ambientes de comunicação, os nós que executam a comunicação têm problemas terminais ocultos porque o alcance das ondas de rádio intervalos são extremamente diferentes. Para evitar a transmissão simultânea, a tecnologia de rede em malha LoRa implementa o método de controle de acesso por divisão de tempo após a sincronização do tempo por GPS. o autor pressupõe-se que todas as estações de rádio operadas no sistema sejam numeradas por ID e o número total também é compreendido, com base no ID, aloca-se dinamicamente o tempo slots que ele pode transmitir. Por exemplo, supondo que o tempo de transmissão por dispositivo na rede sem fio é de 10s (considerando o tempo necessário para recuar para evitar colisões com outros sistemas), ao usar cinco estações sem fio, esses cinco dispositivos não têm nenhum problema com tempo superior a 50s que pode ser transmitido é atribuído como uma transmissão ciclo. Neste ciclo de transmissão, os intervalos de tempo de transmissão são atribuído com base nos respectivos IDs. Como resultado, ocorrência de colisão na comunicação no próprio sistema é evitado. Nesta pesquisa o autor aborda ao projetar adequadamente o fator de dispersão do LoRa, a largura de banda do canal usado e o ciclo de transmissão de acordo com a tecnologia de rede de malha LoRa, avalia a viabilidade de a retransmissão de dados ser feita usando inundações. No entanto, além do mecanismo para evitar a transmissão da mesma informação várias vezes, a fim de reduzir o número de transmissões de inundações enviando informações listando os IDs dos remetentes de sinais recebidos por cada nó no passado como sinais de controle em intervalos regulares, é possível compreender o intervalo dentro do qual seus nós vizinhos podem se comunicar. Quando uma informação nova é recebida, se houver um nó que anuncie  as informações antes de seu próprio horário de transmissão chegar, se a vizinhança o nó chato que ele cobre é adjacente ou se tudo estiver coberto, ele não será retransmitido, como resultado, a retransmissão de informações desnecessárias é suprimida. O autor prototipa um sistema que atualmente implementa esse protocolo baseado no NerveNet desenvolvido pela NTIC,  realizando teste em laboratório. \textcolor{blue}{Neste trabalho, o autor implementa um mecanismo de multiplexação por divisão de tempo, usando sincronismo por GPS, para  evitar colisões. A estrutura exige que cada nó da rede mesh possua GPS para sincronismo. Ao cresecer, deve-se prever timeslots para cada dispositivo da rede isso acarretará  uma latencia maior na rede. Com a premissa de ser uma arquitetura simples, de fácil implemntação e  baixo custo de implantação a  minha arquitetura não implementa nenhum mecanismo de tratamento de colisões, ela deixa a cargo da camada de aplicação o retransmissão por timeout.  }


% Ebi, Christian, et al. "Synchronous LoRa mesh network to monitor processes in underground infrastructure." IEEE Access 7 (2019): 57663-57677.
\textbf{Tag:Trabalho de controle de acesso ao meio e roteamento} Ebi C. \cite{Ebi-19} aborda em sua pesquisa como resolver as limitações do LoRaWAN padrão para atender ambientes complexos, propomos uma nova arquitetura e conceito para controle de acesso médio chamado malha LoRa síncrona . Os principais recursos visíveis são nós repetidores intermediários (RN) que permitam a formação de sub-redes individuais, ou seja,grupos de nós sensores (SN). Os RNs têm ancorar a conectividade LoRaWAN a um gateway e agir como um raiz para nós filho (sensor), posicionados remotamente além da cobertura LoRaWAN. Para esse fim, estendemos a arquitetura LPWAN original de um mero tipo de estrela para uma topologia de malha hierárquica, permitindo uma transmissão multi-hope, assim, obter roteamento mais flexível e extensão cobertura. Ao contrário dos gateways LoRaWAN, os RNs operam em redes e não precisa de acesso à internet. Hardware e firmware de RNs e SNs são idênticos. Ambos funcionam com o mesmo tipo de bateria, mas os nós atendem a diferentes funções operacionais. A comunicação entre um RN e SNs correspondentes são sincronizados com timbres de alta precisão permitindo uma alteração coordenada entre o modo de suspensão e acorde dentro do intervalo de transmissão. A troca de dados entre o LoRaWAN e o síncrono a malha LoRa conta com a mesma tecnologia de camada física, mas parâmetros de transmissão ligeiramente diferentes são usados. Por uma questão de simplicidade, a malha LoRa síncrona usa um fator de propagação fixo e uma potência de transmissão fixa, ambos pode ser configurado antes da implantação dos RNs e SNs. O LoRaWAN e a malha LoRa síncrona usam o formato de pacote LoRa definido pela Semtech, no entanto, diferem quanto à organização da carga útil disponível. LoRaWAN inclui um campo de cabeçalho MAC de um byte (MHDR) na primeira posição contendo informações sobre o tipo de mensagem e usado versão do protocolo. Por outro lado, o formato de carga útil da malha LoRa síncrona é mais simples, um cabeçalho de quadro de cinco bytes contém informações sobre destino, endereço de origem e o tipo do pacote atual(por exemplo, dados ou sincronização), dependendo desse tipo de pacote,a carga contém uma quantidade variável ou fixa de bytes de dados.No caso de um pacote do tipo data , a informação do comprimento é entregue dentro do campo de carga útil. A comunicação dentro da malha LoRa síncrona é baseada no protocolo síncrono LoRa mesh permitindo que os SNs transmitam seus próprios dados, mas também encaminhem pacotes de dados de outros SNs. Mais especificamente, o roteamento O algoritmo impõe o encaminhamento de pacotes de forma dinâmica usando estrutura do tipo de árvore estabelecida com o RN como nó raiz. Isso se aplica ao fluxo de dados nas duas direções, a partir do SN terminal para cima através de outros SNs e do RN para o gateway e reverter a partir do gateway através do RN e outros SNs para o terminal SN (downlink). A comunicação LoRaWAN pode operar dinamicamente na menor taxa possível de dados. No pior dos casos,a carga útil do pacote é limitada a 51 bytes. Um RN comprime dados recebidos de todos os SNs conectados em um único LoRaWAN pacote, portanto, o número de SNs suportados por RN deve exceder a carga útil máxima possível do LoRaWAN. RNs operam como nós raiz de uma sub-rede, os SNs continuam com um processo de ingresso para participar da rede. tem duas maneiras pelas quais SNs não conectados podem ingressar em uma sub-rede:uma junção direta, onde um SN se comunica diretamente com um  RN; ou uma junção indireta, onde um SN não é capaz de alcançar um RN diretamente e o SN tem que se juntar através de outro já SN conectado. Nos dois casos, um SN recém-alimentado verifica primeiro canal para sub-redes existentes. A integração de um SN não conectado a uma sub-rede específica é baseado em sinais transmitidos periodicamente.A partir deste ponto, cada SN é capaz de calcular o tempos de despertar necessários, de acordo com as configurações do ciclo e os horários atribuídos. Esses horários de ativação definem o RTC alarmes, que fazem com que cada SN saia do estado de baixa energia. \textcolor{blue}{Neste trabalho,o autor  usa como base a arquitetura LoRAWAN e propões o inserção de um novo elemento, o roteador intermediário, que conecta em malha um nó sensor ao gateway loRAWAN. Esse nó intemediário também é responsável por  criar sincronimos entre os nós sensores. Tem como ganho o aumento da área de cobertura da rede, porém a latencia é prejudicada, a complexidade de implementação da rede também é um ponto a se destacar.Como ganho a colisão e perda de pacotes é  dimunuida. Se comparado a arquitetura proposta aqui,  essa proposta causa um overhead enorme,  visto que em alguns casos o pacote LORAWAN dispões de apenas 11 bytes de dados. No trabalho desenvolvido como ele não usa como base LoRAWA, esse overhead é  reduzido,  dos 256 bytes de dados permitidos na modulação LoRA,  apenas 16 são utilizados para enderereçemento e roteamento,  ficando disponível  240 bytes em cada pacote para dados. Outro ponto é  que a arquitetura proposta não precisa carregar informação de sincronismo, o que  encarece a rede. }



% Cilfone, Antonio, et al. "Wireless mesh networking: An IoT-oriented perspective survey on relevant technologies." Future Internet 11.4 (2019): 99.
\textbf{Tag:Trabalho de  roteamento} Cilfone A. \cite{Cilfone-19} Dentre as tecnologias LPWAN debatidas pelo autor em sua pesquisa, uma das tecnologias emergentes mais promissoras para aplicativos de IoT é representada pela LoRa(e sua camada MAC denotada como LoRaWAN). Portanto, dentre as muitas atividades de pesquisa relacionadas ao LoRaWAN, um dos últimos aspectos em investigação é a implementação de protocolos de roteamento para trazer recursos de múltiplos saltos ao LoRaWAN. Em geral, o número considerado de saltos é limitado, devido à alta cobertura intrínseca capacidade do LoRa. Em sua pesquisa os autores propõem e avaliam uma camada MAC alternativa para LoRa (chamada LoRa Blink), permitindo a comunicação multi-hop em uma rede de baterias e ciclos de serviço dispositivos. Em seu trabalho, os autores assumem que a rede é caracterizada por uma baixa intensidade espacial de nós, baixo tráfego de dados, um pequeno número de nós (ou seja, não mais que 6). O protocolo integra MAC e roteamento em um único protocolo simples. Sincronização de tempo entre nós é usado para definir o acesso ao canal com fenda. Os nós transmitem simultaneamente nos slots e as propriedades da camada LoRa PHY garantem que apenas uma das transmissões simultâneas seja recebida.As mensagens são distribuídas do coletor para os nós usando a inundação. As mensagens dos nós no coletor usam uma bordagem de inundação direta. Eles usam beacons para sincronização e dividem o tempo em tempo. Cada a tempo contém: slots de sinalização N B , usados para enviar informações sobre a distância do salto e slots de dados N D, que carregam os dados reais. O desempenho do sistema proposto foi avaliado em um pequeno cenário de escala (a distância máxima em 1 salto é 269 m, enquanto em 2 saltos é de cerca de 300 m [74]), e as A taxa de entrega de pacotes (PDR) é da ordem de 80\%. Outra abordagem promissora para o desenvolvimento de protocolos de roteamento para o LoRaWAN, ainda em conformidade com as especificações LoRaWAN, baseia-se em algoritmos conhecidos já disponíveis para outras tecnologias de rádio (por exemplo, AODV ou HWMP, usadas em redes IEEE 802.11). No [75], O HWMP é usado como base para um novo protocolo de roteamento para redes baseadas em LoRa. Em sua implementação, o cabeçalho LoRaWAN MAC é mantido em sua versão original, para que o pacote seja reconhecido como um pacote LoRaWAN; as únicas modificações em relação aos campos MType e RFU, convenientes para identificar o protocolo de roteamento desenvolvido.
\textcolor{blue}{Neste trabalho,o autor  usa como base  o pacote da arquitetura LoRAWAN e propões o inserção de um novo protocolo de roteamento como paylod do pacote LoRWAN para que seja possível realizar comunicação entre senores com uma arquitetura em malha, mas também se mantenha a compatibilidade com a rede LoRAWA, Implementa um mecanismo de sincronimo para diminuir colisões.O protocolo  desenvolvido permite redes em malha de no máximo 6 nós. A  arquitetura proposta  por mim,  não mantém compatibilidade com a rede LoRAWAN, característica que consegue ser atendida no trabalho de Cilfone A.(2019). Porém necessita de um mecanismo complexo de sincronismo por timeslot, tem o overhead que é maior se comparado a rede mesh pura  com o protocolo BABEL modificado. Cilfone A.(2019) também implementa retransmissão por inundação, o que pode interferir no desempenho da rede }

% Huh, Heon, and Jeong Yeol Kim. "LoRa-based Mesh Network for IoT Applications." 2019 IEEE 5th World Forum on Internet of Things (WF-IoT). IEEE, 2019.
\textbf{Tag:Trabalho de controle de acesso ao meio e roteamento} Huh H. \cite{Huh-19} Para resolver os problemas associados ao padrão Lo-RaWAN, quando empregado em redes privadas ad-hoc o autor desenvolveu uma pilha de protocolo LoRa modificada que suporta malha rede e acesso múltiplo por divisão de tempo. Porque topologias de rede convencional, como topologias de estrela e árvore, são bem estabelecidos, altamente padronizados e neutros ao fornecedor, eles são frequentemente usados para redes públicas. Para superar os problemas mencionados acima, o autor propoe remover o gateway e os nós finais vizinhos da tabela de malha e coloque o nó final, em cima da tabela de malha seu protocolo LoRa modificado, o autor apresentada as características da malha proposta: 
\begin{itemize}
    \item  Não há necessidade de planejamento de célula com os gateways, e os nós finais podem ser implantados de forma relativamente simples e flexível
    \item Os caminhos de roteamento são estabelecidos automaticamente entre os nós finais. Se houver uma falha no roteamento existente caminho, o redirecionamento é feito na rede e novos caminhos são reconfigurados.
    \item A rede é otimizada para comunicação de baixa taxa embandas ISM sub-GHz.
    \item As comunicações bidirecionais N: 1 e 1: N são possíveis.
    \itemA rede é adequada para medição inteligente, construção de sistemas de gerenciamento de energia (SGA) e monitoramento de segurança em campos de construção
\end{itemize}

Para sistemas que possuem muitos nós finais em menos de um salto (área de cobertura direta) e precisa coletar dados orientados a eventos em vez de pesquisar, o autor desenvolve uma pilha TEDS para reduzir a taxa de colisão de dados. Isso evita o aumento simultâneo de a carga devido a sinais de processamento de eventos e corrupção de dados.Em particular, é adequado para medição remota de água / gás sistemas que operam com bateria, sistemas de combate simulados que requerem recursos quase em tempo real e controle de iluminação pública isso requer resposta rápida de muitos nós. O auto também desenvolve um gateway para o protocolo LoRa proposto com enfatizando as vantagens:
\begin{itemize}
    \item Aplicável à maioria dos cenários de operação de IoT.
    \item Suporta no máximo quatro canais LoRa (nó finalmalha de rede).
    \item Backhaul sem fio adicional com freqüência de 38,4 kbps chaveamento por turnos (FSK).
    \item Ethernet (conexão WAN)
    \item Uso interno e externo (design à prova de água / poeira).
\end{itemize}
O autor conclui sua pesquisa com a apresentação de três caso de uso da proposta de protocolo LoRa, que pode ser implementado em uma rede privada trabalhos. 
\textcolor{blue}{Neste trabalho,o autor desenvolve um protocolo de roteamente mesh novo para  substituir o LoRAWA ( como o do meu trabalho) ele  usou o LoRa  com esse protocolo para desenvolver o que chamou de redes privadas LoRA. Não tem muito detalhe osbre frquencias, SF. Ele  fala em um  mecanismo chamado pilha TEDS, para  diminuir a colisão.O artigo  focou no desenvolvimento do  e gateway para essa rede privada onde monta um gateway com backhaul  ethernet. A proposta do meu trabalho  vai na mesma linha, mas ele usa para coleta de dados apenas. No meu caso, a rede é usada para controle ou seja é uma rede que tem a mesma capacidade de TX e RX. Também não implemento mecanismo de controle de colisão. A grande diferença é o aumento do throughput  da minha rede, pois implemento multiplexação de frequencias ( pacote particinado e enviado por dois canais ao mesmo tempo) isso diminui latência e colisão }
